Tractable Diversity: Scalable Multiperspective Ontology Management via Standpoint EL

The tractability of the lightweight description logic EL has allowed for the construction of large and widely used ontologies that support semantic interoperability. However, comprehensive domains with a broad user base are often at odds with strong axiomatisations otherwise useful for inferencing, since these are usually context-dependent and subject to diverging perspectives. In this paper we introduce Standpoint EL, a multi-modal extension of EL that allows for the integrated representation of domain knowledge relative to diverse, possibly conflicting standpoints (or contexts), which can be hierarchically organised and put in relation to each other. We establish that Standpoint EL still exhibits EL's favourable PTime standard reasoning, whereas introducing additional features like empty standpoints, rigid roles, and nominals makes standard reasoning tasks intractable.

==> sections/EL-proofs3.tex <==
\subsection{Preliminaries}
\textcolor{red}{Clarify what are subformulas and clarify that here we are using $\kb = TBox \cup ABox \cup SBox$ .}

\begin{definition}[Subformula]
    Let us define a subformula $\phi$ of a knowledge base $\kb$ in the following way,
    \begin{itemize}
        \item For all $\phi\in\kb$, $\phi$ is a subformula of $\kb$, and
        \item if $\standbs\phi$ is a subformula, then $\phi$ is also a subformula.
    \end{itemize}
\end{definition}

\noindent Given a Knowledge Base $\kb$, denote by
\begin{itemize}[leftmargin=0.8cm]
    \item $\BCC$ (\define{basic concepts}) the set of concept names used in $\kb$, together with $\top$.
    \item $\CC$  the set of concepts occurring in $\kb$, with $\BCC\subseteq\CC$.
    \item $\SC$  the set of standpoint symbols occurring in $\kb$, together with $*$.
    \item $\forC$ the set of subformulas of $\kb$.
    \item $\objC$ the set of all individual names occurring in $\kb$.
\end{itemize}
\vspace{0.5em}

We use $C, D, \ldots \in \CC$ to denote concepts, $\phi, \psi, \ldots \in \forC$ to denote formulas, $a, b, \ldots \in \objC$ to denote individuals and $\Phi, \Psi, \ldots \in \forC\cup\CC\cup\objC$ to denote either.

\begin{definition}[Size]
    Let us define the size of a knowledge base $\kb$, denoted by $\size{\kb}$ as
    $$ \size{\kb} \eqdef \card{\forC} + \card{\CC} + \card{\SC} $$
\end{definition}


%\textcolor{red}{SR: I assumed we had agreed the $+ \card{\objC}$ wouldn't be necessary?}
%\hs{This implicitly mixes ABox and CBox. I would prefer to treat them separately because ABox normalisation is essentially one-step and moves complex concepts entirely into the CBox.}
%\hs{The form “$C\dlsub D$” is actually “$\standball[C\dlsub D]$” and is therefore covered by the form “$\standbs[C\dlsub D]$”, so is it needed in this explicit form?}
\begin{definition}[Normal form]

    Let us define the assumed normal form of the formulas of a knowledge base $\kb$ as
    \begin{align*}
        \st          & \preceq \sp      \\
        %		C              & \sqsubseteq  D   \\
        \standb{s}	[	C & \sqsubseteq  D ] \\
        %		C_1            & (x)              \\
        \standb{s}	[A & (x)]             \\
        %		R              & (x,y)            \\
        \standb{s}	[R & (x,y)]
    \end{align*}

    Where $C$ is of the form $A$, $\exists R.A$ or $A \sqcap B$ with $A, B \in\BCC$ and $D$ is of the form $E$,  $\exists R.E$, $\standds E$ or $\standbs E$ with $E \in\BCC\cup\{\bot\}$
\end{definition}


\subsection{A Tableau for Standpoint-$\EL$}

Let us present a tableau algorithm to build a quasi-model for Standpoint $\EL$. We recall that for modal logic extensions of $\mathcal{ALC}$ with constant domains, it has been shown that models can be represented as quasi-models. Our case cannot be treated in precisely the same way, as we need to take greater care to show tractability in the end, however similar ideas can be employed. Compared to classical quasi-models, we follow a dual approach: rather than building a quasi-model from a tree of quasi-worlds, we will build a \emph{quasi-model} from a set of \emph{quasi (domain) elements}, where each of the latter consists of assembled information regarding one individual's specifics in each world. We begin with some definitions.

Let us define formally what we mean by a constraint system for a given standpoint $\EL$-knowledge base $\kb$.
A \emph{constraint} for $\kb$ is an atom of the form $x\col C$, $x\col a$, $x\col \phi$ or $x\col \st$, where $x$ is a variable, $C\in \CC$ a concept, $a\in \objC$ an individual, $\st \in \SC$ a standpoint symbol and $\phi\in\forC$ is a formula.
\emph{Constraint systems} are finite sets of constraints.

\begin{definition}[Initial Constraint System for $\kb$]\label{def:ini-constraint-system}
    The \emph{initial constraint system} for $\kb$, called $\initialcs$, is the set
    $$ \{(x_{\st}\col *), (x_{\st}\col \top), (x_{\st}\col \phi),  (x_{\st}\col \st) \mid \phi\in\kb, \st\in\SC \}$$
\end{definition}

\begin{definition}[Constraint System for $\kb$]\label{def:constraint-system}
    A \emph{constraint system} $S$ for $\kb$ is a finite set of constraints for $\kb$ such that
    \begin{enumerate}
        \item $\initialcs\subseteq S$ and
        \item for each variable $v$ in $S$, $(v\col *)\in S$ and $(v\col \top)\in S$.
    \end{enumerate}

\end{definition}

A variable is called \emph{fresh} if it does not (yet) occur in $S$.
Let $\stvar{S}{\st} := \{v \mid (v\col \st)\in S\}$ denote the set of $\st$-variables in $S$ and $\stlabel{S}{v}=\{\st\mid(v\col \st)\in S\}$ the `standpoint signature' of $v$ in $S$.

Given the rules specified in Fig. \ref{fig:rules}, we say that a constraint system $S$ is \emph{complete} if no local completion rule is applicable to $S$.
Local completion rules operate exclusively on constraint systems, while global rules operate on completion graphs (defined below), i.e. they involve more than one constraint system.

\begin{definition}[Element label]\label{def:element-label}
    An element label $L$ is a set of triples $(C,s,x)\in L$ where $C\in\BCC$ is a concept, $s\subseteq\SC$ is a set of standpoints and $x$ is a variable.
\end{definition}

\begin{definition}[Quasi-role]\label{def:quasi-role}
    A \emph{quasi-role} is a tuple $\langle \qelem, v, \qelem', v', R\rangle$ where $\qelem$ and $\qelem'$ are elements, $v$ and $v'$ are variables and $R$ is a role name in $\kb$.
\end{definition}

\begin{definition}[Completion Graph]\label{def:completion-set}
    A \emph{completion graph} for a $\SEL$ knowledge base $\kb$ is a tuple $\mathbf{CG}=\tuple{\Delta,\consisf,\elabelf,\rolesf}$, with $\Delta$ a non-empty set of elements; $\consisf$ a function mapping each $\qelem\in\Delta$ to a constraint system $\consis{\qelem} = S_{\qelem}$ for $\kb$; $\elabelf$ a map from $\Delta$ into element labels; and $\rolesf$ a set of quasi-roles such that
    \begin{itemize}
        \item for all $\langle \qelem, v, \qelem', v', R\rangle\in\rolesf$, it holds that %$\qelem,\qelem'\in\Delta$ and 
              $(v\col \st)\in \consis{\qelem}$ iff $(v'\col \st)\in \consis{\qelem'}$, and
        \item if $(C,s,x)\in\elabel{\qelem}$, then $\{x\col C\}\cup \{x\col \st\mid \st\in s\}\subseteq \consis{\qelem}$.
              %        \item for each $a\in\objC$ there is a unique element $\qelem_a\in\Delta$ such that $(v\col a)\in\consisu{\qelem_a}$ for all variables $v$ in $\consisu{\qelem_a}$.
              %  \item for each locally complete $\consis{\qelem}$ and $\consis{\qelem}$, $\{ \stlabel{\qelem}{v} \mid v \in\stvar{\qelem}{*}\}=\{ \stlabel{\qelem'}{v} \mid v \in\stvar{\qelem'}{*}\}$ 
              %       \item \textcolor{red}{for each locally complete $\consis{\qelem}$ and $\consis{\qelem'}$, if $(v\col\phi)\in\consis{\qelem}$ then there is some $v'$ such that $\stlabel{\qelem}{v}=\stlabel{\qelem'}{v'}$ and $(v'\col\phi)\in\consis{\qelem'}$}
    \end{itemize}
    % \textcolor{blue}{S.R.: The last two bullet points are not satisfied at all times during the tableau algorithm. So technically, the data structure we are working with stops being a ``completion graph'' for certain periods, which seems odd. I'd prefer to define an extra property (say ``homogenous'') that is satisfied for a completion graph whenever these two bullet points are satisfied.}\textcolor{purple}{L.G.: Fair enough. On the last point I phrased it specifying that this is only the case when they are locally complete, precisely to avoid that , but an additional property may look better indeed.}  
\end{definition}

For convenience of presentation, we use the shortcut $\stvar{\qelem}{\st}$ for $\stvar{\consis{\qelem}}{\st}$ and $\stlabel{\qelem}{v}$ for $\stlabel{\consis{\qelem}}{v}$.
%\textcolor{blue}{S.R.: These abbreviations are already used in the definition above...}\textcolor{purple}{L.G.: I know... I thought I could get away with it because it is right after and it looks very cluttered without the abbreviation, but I guess it's better to go with the full version.}  
Similarly, for any $\mathbf{CG}=\tuple{\Delta,\consisf,\elabelf,\rolesf}$, we will refer to all $\qelem\in\Delta$ simply as elements (or quasi-elements) of $\mathbf{CG}$.

$\mathbf{CG}$ is said to be \emph{locally complete} if for every element $\qelem$ in $\mathbf{CG}$, $\consis{\qelem}$ is complete. We call $\consis{\qelem}$ \emph{globally complete} if no global completion rule (see Fig.~\ref{fig:rules}) is applicable to $\consis{\qelem}$ in $\mathbf{CG}$, and we call $\mathbf{CG}$ \emph{globally complete} if it is \emph{locally complete} and no global completion is applicable to  $\mathbf{CG}$ as a whole.

\begin{definition}[Coherence]\label{def:coherence}
    A completion graph $\mathbf{CG}=\tuple{\Delta,\consisf,\elabelf,\rolesf}$ for $\kb$ is \emph{coherent} if it satisfies the following conditions,
    \begin{itemize}
        \item for each $a\in\objC$ there is a unique element $\qelem_a\in\Delta$ such that $(v\col a)\in\consisu{\qelem_a}$ for all variables $v$ in $\consisu{\qelem_a}$,
        \item for each $v$ in $\consis{\qelem}$, every $\consis{\qelem'}$ contains some $v'$ such that $\stlabel{\qelem}{v}=\stlabel{\qelem'}{v'}$, and
        \item for each $\consis{\qelem}$ and $\consis{\qelem'}$, if $(v\col\phi)\in\consis{\qelem}$ then $(v'\col\phi)\in\consis{\qelem'}$ for all $v'$ with $\stlabel{\qelem}{v}=\stlabel{\qelem'}{v'}$.
              %\item \textcolor{orange}{for each $\tuple{\qelem, v, \qelem', v', R}\in\rolesf$ with $(v'\col C)\in\consisu{\qelem'}$, we have $(v \col \exists R.C) \in\consisu{\qelem}$ in case $\exists R.C \in\CC$.}
    \end{itemize}
    %\textcolor{blue}{S.R.: The 4th bullet point is redundant, IMHO, because it seems to coincide with being closed under $\mathbf{R}_{\downarrow}$.}\\
    %\textcolor{blue}{S.R.: Is ``homogenous'' a good term? Maybe "coherent" is better?}
\end{definition}

\begin{definition}[Clash]
    A constraint system $S$ contains a \emph{clash} if $x\col \bot \in S$ for a variable $x$. Otherwise, we call $S$ \emph{clash-free}.
    %
    A completion graph $\mathbf{CG}$ contains a \emph{clash} if $\consis{\qelem}$ contains a clash for some $\qelem \in \mathbf{CG}$. Otherwise, $\mathbf{CG}$ is called \emph{clash-free}.
\end{definition}

\subsubsection{The algorithm}

To decide whether a given $\SEL$ knowledge base $\kb$ in normal form is satisfiable, we form the initial completion graph $\mathbf{CG}_\kb$ with $\rolesf=\emptyset$ and $\Delta$ consisting of an element $\qelem_{\top}$ with $\elabel{\qelem_{\top}}=\emptyset$ and $\consis{\qelem_{\top}}=\initialcs$
and for every $a\in\objC$, an element $\qelem_a$ with $\elabel{\qelem_{a}}=\emptyset$ and $\consis{\qelem_{a}}$ set to
$$ \initialcs \cup \{(x_{\st}\col a)\mid x_{\st}\in\stvar{\initialcs}{*} \}$$
For the sake of intuition, we can think of $\qelem_{\top}$ as the constraint system for an individual $d\in\Delta$ with $\allstandb\top(d)$ and for every $a\in\objC$, $\qelem_{a}$ is the constraint system for that named individual.
Notice that the initialisation of a variable for each standpoint in the initial constraint system guarantees non-empty standpoints.

After that, we repeatedly apply the local and global completion rules from Fig.~\ref{fig:rules} in the order specified in the pseudo-code of Fig.~\ref{fig:pseudocode}

\begin{figure}
    \begin{mdframed}
        \paragraph{Tableau completion rules} (Assume $C \in\CC\cup\{\bot\}$)

        \begin{itemize}
            \item Local labelling (LL) rules:
                  \begin{enumerate}[leftmargin=0.5cm, itemsep=0.5em]
                      \item[$\mathbf{R}_{\preceq}$] If $\{x \col \st,\ x' \col \st\preceq \sp\}\subseteq S$ but $(x \col \sp) \notin S$, then set $S:=S\cup \{x \col \sp\}$
                  \end{enumerate}
            \item Local non-generating (LN) rules:
                  \begin{enumerate}[leftmargin=0.5cm, itemsep=0.5em]
                      \item[$\mathbf{R}_\sqcap$] If $\{x \col C,\ x \col D\}\subseteq S$, $(x \col C\sqcap D)\notin S$ and $C\sqcap D\in\CC$, then set $S:=S\cup \{x \col C \sqcap D\}$
                      \item[$\mathbf{R}_\sqsubseteq$] If $\{x \col C,\  x \col C\sqsubseteq D\}\subseteq S$ but $(x \col D)\notin S$, then set $S:=S\cup \{x \col D\}$
                      \item[$\mathbf{R}_{\Box}$] If $\{x \col \!\standbs\Phi,\  x' \col \st\}\subseteq S$ but $(x' \col \Phi)\notin S$, then set $S:=S\cup \{x' \col \Phi\}$
                      \item[$\mathbf{R}_{g}$] If $\{x \col \mathbf{G}\}\subseteq S$ but $(x' \col \mathbf{G})\notin S$, then set $S:=S\cup \{x' \col \mathbf{G}\}$
                      \item[$\mathbf{R}_{a}$] If $\{x \col a,\ x \col C(a)\}\subseteq S$ but $(x \col C)\notin S$, then set $S:=S\cup \{x \col C\}$
                  \end{enumerate}

            \item Local generating (LG) rule:
                  \begin{enumerate}[leftmargin=0.5cm, itemsep=0.5em]
                      \item[$\mathbf{R}_{\Diamond}$] If $(x \col \standds C)\in S$ and $\{x' \col \st,\ x' \col C\}\nsubseteq S$ for all $x'$ in $S$, then create a fresh variable $x'$ and set $S:=S\cup \{x'\col C,\ x'\col \st,\ x'\col *,\ x'\col \top\}$.
                  \end{enumerate}
            \item Global non-generating (GN) rules:
                  \begin{enumerate}[leftmargin=0.5cm, itemsep=0.5em]
                      \item[$\mathbf{R}_{\downarrow}$] If %$(x \col \exists R.C)\in \consis{\qelem}$ and 
                          $(x\col C)\in \consis{\qelem}$ %for some $\qelem'\in\Delta$ 
                          and $\langle \qelem', x', \qelem, x, R\rangle\in\rolesf$, but $(x' \col \exists R.C)\notin \consis{\qelem'}$ \textcolor{blue}{despite $\exists R.C\in\CC$}, then set $\consis{\qelem'}:=\consis{\qelem'}\cup \{x' \col \exists R.C\}$.

                      \item[$\mathbf{R}_{r}$] If $\{x \col a,\ x \col R(a,b)\}\subseteq \consis{\qelem}$ but $\langle \qelem, x, \qelem', x, R\rangle\notin\rolesf$ for some $\qelem'\in\Delta$ with $(x'\col b)\in\consis{\qelem'}$, then set $\consis{\qelem'}:=\consis{\qelem'}\cup \{x \col \top\}\ \cup\ \{x\col \st \mid \st\in\stlabel{\qelem}{x} \}$ and $\rolesf:=\rolesf\cup \{\langle \qelem, x, \qelem', x, R\rangle\}$.

                      \item[$\mathbf{R}_{r'}$] If $\{x \col b,\ x \col R(a,b)\}\subseteq \consis{\qelem}$ but $\langle \qelem', x, \qelem, x, R\rangle\notin\rolesf$ for some $\qelem'\in\Delta$ with $(x'\col a)\in\consis{\qelem'}$, then set $\consis{\qelem'}:=\consis{\qelem'}\cup \{x \col \top\}\ \cup\ \{x\col \st \mid \st\in\stlabel{\qelem}{x} \}$ and $\rolesf:=\rolesf\cup \{\langle \qelem', x, \qelem, x, R\rangle\}$.

                      \item[$\mathbf{R}_{\exists'}$] If there are some $\qelem,\qelem' \in\Delta$ with $(x \col \exists R.C)\in \consis{\qelem}$, $(C,\stlabel{\qelem}{x},x')\in\elabel{\qelem'}$ and $\qelem\neq\qelem'$ or $x=x'$, but $\langle \qelem, x, \qelem'', x'', R\rangle\notin\rolesf$ for all $\qelem'', x''$ with $(C,\stlabel{\qelem}{x},x'')\in\elabel{\qelem''}$ and $\qelem\neq\qelem''$ or $x=x''$, then set $\rolesf:=\rolesf\cup \{\langle \qelem, x, \qelem', x', R\rangle\}$.
                  \end{enumerate}
            \item Global generating (GG) rule:
                  \begin{enumerate}[leftmargin=0.5cm, itemsep=0.5em]
                      \item[$\mathbf{R}_{\exists}$] If there is some $\qelem \in\Delta$ with $(x \col \exists R.C)\in \consis{\qelem}$, but there is no $\qelem'$ with $(C,\stlabel{\qelem}{x},x')\in\elabel{\qelem'}$, $\langle \qelem, x, \qelem', x', R\rangle\in\rolesf$ and either $\qelem'\neq\qelem$ or $x'=x$, then create a new element $\qelem'$ as well as a fresh variable $x'$, set $\elabel{\qelem'}=\{(C,\stlabel{\qelem}{x},x')\}$, $\rolesf:=\rolesf\cup \{\langle \qelem, x, \qelem', x', R\rangle\}$, and let $\consis{\qelem'}$ be the union of
                          $$ \initialcs\ \cup\ \{x'\col C,\ x'\col \top\}\ \cup\ \{x'\col \st \mid \st\in\stlabel{\qelem}{x} \}$$
                  \end{enumerate}
        \end{itemize}
    \end{mdframed}

    \caption{The completion rules for the tableau. $\mathbf{G}$ can be of the form $a$, $(\st\preceq\sp)$ and $\standbs \phi$, all of which share the property of applying globally to all precisifications in a model. \textcolor{blue}{S.R.: FWIW, in the presence of $\mathbf{R}_{g}$, the rules $\mathbf{R}_{\preceq}$ and $\mathbf{R}_{\Box}$ could be ``localized'' even more, so they speak of only one variable $x$. But it also works as is.}} \label{fig:rules}
\end{figure}

\begin{figure}
    \begin{mdframed}

        \begin{lstlisting}[basicstyle=\rmfamily,morekeywords={if,define,procedure,then,return},keywordstyle=\rmfamily\bfseries]
define procedure sat(CG):
  if CG contains a clash 
    then return unsatisfiable;
  if a LL rule r is applicable to CG:	
    then apply r to CG; return sat(CG)
  if a LN rule r is applicable to CG:
    then apply r to CG; return sat(CG)
  if a LG rule r is applicable to CG:	
    then apply r to CG; return sat(CG)
  if a GN rule r is applicable to CG:
    then apply r to CG; return sat(CG)
  if a GG rule r is applicable to CG:
    then apply r to CG; return sat(CG)
  return satisfiable
		\end{lstlisting}
    \end{mdframed}
    \caption{The satisfiability checking algorithm for $\SEL$}\label{fig:pseudocode}
\end{figure}

\subsubsection{Quasi-structures and Quasi-models}
This section shows how $\SEL$ models can be represented in a particular form of (dual) quasi-models. We characterise our version of quasi-models syntactically similar to Lutz et~al. %quasi-models
The usual quasi-model constructions that can be found in the literature consist of a set of quasi-worlds and a relation over these quasi-worlds.
Instead, our construction is based on a set of quasi-elements that characterise the constant domain and its interpretation in the different precisifications.

\begin{definition}[Run]\label{def:run}
    Let $\mathbf{CG}=\tuple{\Delta,\consisf,\elabelf,\rolesf}$ be a completion graph for $\kb$. Then, a \emph{run} $r$ in $\mathbf{CG}$ is a map associating each element $\qelem\in\Delta$ to a variable $r(\qelem)\in \stvar{\qelem}{*}$ in such a way that
    \begin{enumerate}[leftmargin=0.5cm, itemsep=0.5em, label={\rm C\arabic*}, ref={(C\arabic*)}]
        \item if $(r(\qelem)\col \st)\in\consisu{\qelem}$, then $(r(\qelem')\col \st) \in \consisu{\qelem'}$  for all $\qelem,\qelem'\in\Delta$ and $\st\in\SC$,\label{condition:run-standpoint}
        \item if $\tuple{\qelem, v, \qelem', v', R}\in\rolesf$ and $r(\qelem)=v$, we have $r(\qelem')=v'$, and %, \textcolor{purple}{and $(v \col \exists R.C) \in\consisu{\qelem}$ if $(v'\col C)\in\consisu{\qelem'}$}
              \label{condition:run-role}
              %\textcolor{blue}{S.R.: The purple part is not a constraint on $r$ but rather another ``homogeneity'' constraint on completion graphs.}            
        \item if $(r(\qelem)\col \exists R.C) \in\consisu{\qelem}$, there is a $\qelem'\in\Delta$ with $\tuple{\qelem, r(\qelem), \qelem', r(\qelem'), R}\in\rolesf$ and $(r(\qelem')\col C) \in\consisu{\qelem'}$. \label{condition:run-existential}
              %            \item if $(r(\qelem)\col \phi)\in\consisu{\qelem}$, then $(r(\qelem')\col \phi) \in \consisu{\qelem'}$ for all $\qelem'\in\Delta$. \textcolor{orange}{This should also be redundant by coherence.} \label{condition:run-axiom}
    \end{enumerate}
\end{definition}

\begin{definition}[Quasi-model]\label{def:quasi-model}
    A \emph{quasi-model} of $\kb$ is defined to be a tuple $\mathcal{Q}=\tuple{\Delta,\consisfu,\elabelf,\rolesf,\runsf}$ where $\tuple{\Delta,\consisf,\elabelf,\rolesf}$ is a globally complete, coherent and clash-free completion graph for $\kb$, and $\runsf$ a set of runs in $\tuple{\Delta,\consisf,\elabelf,\rolesf}$ such that
    for every $\qelem\in\Delta$ and variable $v\in \stvar{\qelem}{*}$, there exists a run $r$ in $\runsf$ such that $r(\qelem)=v$. $\kb$ is called \emph{quasi-satisfiable} iff $\kb$ has a quasi-model.
\end{definition}



\begin{theorem}\label{theorem:satisfiable-iff-quasisatisfiable}
    A $\SEL$ KB in NNF is satisfiable iff it is quasi-satisfiable.
\end{theorem}

\begin{proof}
    ($\Rightarrow$) Suppose $\kb$ is satisfiable. Then there is a model $\dlstruct = \tuple{\Dom, \Precs, \sigma, \gamma}$ such that $\dlstruct\models\kb$ from which we will construct a quasi-model $\mathcal{Q}=\tuple{\Delta,\consisfu,\elabelf,\rolesf,\runsf}$ of $\kb$, using the same domain $\Delta$.

    % For all $\pi\in\Pi$ and $\qelem\in\Dom$, we let

    %	$$ \tau^{\gamma(\pi)}(\qelem) = \{ C \in \CC \mid \qelem\in C^{\gamma(\pi)}\}$$        %%% NOT NEEDED

    Now, for each domain element $\qelem\in\Dom$ define a constraint system $\consisu{\qelem}$ with an individual variable for each precisification and a variable for each standpoint (i.e. $\stvar{\qelem}{*} =\{v_{\pi} \mid \pi\in\Pi \} \cup \{v_{\st} \mid \st\in\SC \}$). We let $\consisu{\qelem}$ contain the following sets of constraints:
    $$ \{v_{\pi}\col C \mid \qelem \in C^{\gamma(\pi)}, \pi\in\Pi\}\cup \{v_{\pi}\col a \mid \qelem=a^{\gamma(\pi)}, \pi \in \Pi\}  $$
    $$\cup\ \{v_{\pi}\col \phi \mid \dlstruct, \pi\models \phi,\ \phi\in\forC\} \cup\ \{v_{\pi}\col \st \mid \pi\in\sigma(\st)\}$$
    and the following constraints for each $v_{\st}$ (with $\st\in\SC$), which are a copy of some $\pi_{\st}\in\sigma(\st)$:
    $$ \{v_{\st}\col C \mid \qelem \in C^{\gamma(\pi_{\tiny\st})}\}\cup \{v_{\st}\col a \mid \qelem=a^{\gamma(\pi_{\tiny\st})}\} $$
    $$\cup\ \{v_{\st}\col \phi \mid \dlstruct, \pi_{\st}\models \phi,\ \phi\in\forC\}  \cup\ \{v_{\st}\col \sp \mid \pi_{\st}\in\sigma(\sp)\}$$
    Notice that the constraints for the variable $v_{\st}$ are exactly the same as for $v_{\pi_{\tiny\st}}$, already in $\consisu{\qelem}$.

    As for the element labels associated with $\qelem$, we let $\elabel{\qelem}$ be the set satisfying the following property: for each $\exists R.C \in\CC$, if $\qelem'\in(\exists R.C)^{\gamma(\pi)}$, $(\qelem',\qelem)\in R^{\gamma(\pi)}$ and $\qelem\in C^{\gamma(\pi)}$, then $(C,s,v_{\pi})\in\elabel{\qelem}$ with $s=\{\st\in\SC \mid \pi\in\sigma(\st)\}$. Notice that each $v_{\st}$ is a duplicate of a $v_{\pi}$ hence no special consideration is needed. For the quasi-roles, we let $\tuple{\qelem, v_{\pi}, \qelem', v_{\pi}, R}\in\rolesf$ if $(\qelem,\qelem')\in R^{\gamma(\pi)}$.

    Finally, define a set of runs $\runsf$ containing one run $r_{\pi}$ for every precisification $\pi\in\Pi$ and another for every standpoint $\st\in\SC$, such that
    $$ r_{\pi}(\qelem) = v_{\pi} \qquad \text{and} \qquad r_{\st}(\qelem) = v_{\st}$$

    %%%%%%%% PROOF

    We now show that $\mathcal{Q}=\tuple{\Delta,\consisfu,\elabelf,\runsf}$ is a quasi-model for $\kb$. First, note that for each domain element $\qelem\in\Delta$, $\elabelf(\qelem)$ is a set of element labels and $\consisu{\qelem}$ a constraint system. Moreover, since $\dlstruct$ is a model, then $\consisu{\qelem}$ is clash-free. Of each $\consisu{\qelem}$, it remains to show that it is a constraint system for $\kb$ and that it is globally complete. Recall that $\dlstruct$ is a model and that $\kb$ is in normal form; Assume w.l.o.g. that $v_{\st}$ is a shortcut for $v_{\pi_{\st}}$ which corresponds to the precisification $\pi_{\st}$.

    %%%%%%%%%%%%% EACH CONSTRAINT SYSTEM IS A "CONSTRAINT SYSTEM FOR K" AND IT IS COMPLETE AND CLASH FREE
    \begin{itemize}
        \item $\consisu{\qelem}$ is a constraint system for $\kb$:
              \begin{itemize}
                  \item We have $(v\col *)\in S$ and $(v\col \top)\in S$ for each variable $v$ in $\consisu{\qelem}$ by construction  because $\sigma(*)=\Pi$ and ${\top}^{{\gamma(\pi)}}=\Dom$ for all $\pi\in\Pi$.
                  \item We have constructed one variable $v_{\st}$ (for each $\st\in\SC$) with $\{v_{\st}\col \sp \mid \pi_{\st}\in\sigma(\sp)\}$ for some precisification $\pi_{\st}\in\sigma(\st)$. Then, $(v_{\st}\col \sp)\in\consisu{\qelem}$. Notice that by construction also $\{(x_{\st}\col *), (x_{\st}\col \top), (x_{\st}\col \phi)\}\subseteq\consisu{\qelem}$. It is clear that $\initialcs\subseteq\consisu{\qelem}$.
              \end{itemize}
        \item $\consisu{\qelem}$ is globally complete, i.e. no rule is applicable to $\consisu{\qelem}$:
              \begin{itemize}
                  \item By construction, each variable $v_{\pi}$ in $S$ has all the subformulas $\phi\in\forC$ such that $\dlstruct, \pi \models \phi$. The only rule that produces additional axioms is $\mathbf{R}_{\Box}$ and it is not applicable by construction: if $(v_{\pi}\col \standbs \phi) \in S$ and $v_{\pi'}\in\stvar{S}{\st}$ is because $\dlstruct, \pi \models \standbs\phi$ and $\pi'\in\sigma(\st)$. Hence we have $\dlstruct, \pi \models \phi$ and consequently $(v_{\pi'}\col \phi) \in S$.
                  \item The rules $\mathbf{R}_{\sqcap}$, $\mathbf{R}_{\sqsubseteq}$, $\mathbf{R}_{\Box}$ and $\mathbf{R}_{a}$ produce a new concept assignation to a variable $v\in S$. Thus, they correspond to the concept interpretations to which a domain element belongs in one precisification. Since $\dlstruct$ is a model, those concept assignations are already captured in $\tau^{\gamma(\pi)}(\qelem)$ and thus in $\consisu{\qelem}$ by construction.
                  \item $\mathbf{R}_{\preceq}$ is applicable if $(v_{\pi}\col\st\preceq \sp)\in \consisu{\qelem}$ and $v_{\pi'}\in\stvar{\qelem}{\st}$ but $v_{\pi'}\notin\stvar{\qelem}{\sp}$. But if $(v_{\pi}\col \st\preceq \sp)\in \consisu{\qelem}$ then $\dlstruct, \pi \models (\st\preceq \sp)$ and then if $\pi'\in\sigma(\st)$ then $\pi'\in\sigma(\sp)$, thus by construction $v_{\pi'}\in\stvar{\qelem}{\sp}$, i.e. $(v_{\pi'}\col \sp)\in \consisu{\qelem}$. Hence, the rule is not applicable.
                  \item $\mathbf{R}_{g}$ is applicable if $(v_\pi\col \mathbf{G})\in S$ and $(v_\pi'\col \mathbf{G})\notin S$. However, if $\mathbf{G}$ is a named individual we have $a^{\gamma(\pi)}=a^{\gamma(\pi')}$ for all $\pi,\pi'\in\Pi$ and if $\mathbf{G}$ is an axiom of the form $(\st\preceq\sp)$ or $\standbs\phi$ then we have $\dlstruct, \pi\models \mathbf{G}$ iff $\dlstruct, \pi'\models \mathbf{G}$ for all $\pi,\pi'\in\Pi$. Thus $(v_\pi'\col \mathbf{G})\in S$ and the rule is not applicable.
                  \item $\mathbf{R}_{\Diamond}$ is applicable if $\{v\col \standds C\}\in\consisu{\qelem}$ and $\{v'\col C\}\notin \consisu{\qelem}$ for all $v'\in\stvar{\qelem}{\st}$. However, if $\{v\col \standds C\}\in\consisu{\qelem}$ then there must be some precisification $\pi\in\Pi$ in which $\qelem \in (\standds C)^{\gamma(\pi)}$, which means that there must be some $\pi'\in\sigma(\st)$ such that $\qelem \in C^{\gamma(\pi')}$, and thus by construction there is some $v'$ such that $\{v'\col C,\ v'\col \st\}\subseteq\consisu{\qelem}$, hence $\mathbf{R}_{\Diamond}$ is not applicable.
                  \item $\mathbf{R}_{\downarrow}$ is applicable if
                        $(x'\col D)\in \consis{\qelem'}$ and $\langle \qelem, v_{\pi}, \qelem', x', R\rangle\in\rolesf$, but $(v_{\pi} \col \exists R.D)\notin \consis{\qelem}$. By construction we have $\langle \qelem, v_{\pi}, \qelem', x', R\rangle\in\rolesf$ only if $(\qelem,\qelem')\in R^{\gamma(\pi)}$ and $x'=v_{\pi}$. Since $\dlstruct$ is a model then for all $D\in\BCC$ if $\qelem'\in D^{\gamma(\pi)}$ and $(\qelem,\qelem')\in R^{\gamma(\pi)}$, then $\qelem\in \exists R.D^{\gamma(\pi)}$. Thus by construction if $(v_{\pi}\col D)\in \consis{\qelem'}$, then $(v_{\pi} \col \exists R.C)\in \consis{\qelem}$ and the rule is not applicable.

                  \item $\mathbf{R}_{r}$ is applicable if $\{v_{\pi} \col a,\ v_{\pi} \col R(a,b)\}\subseteq \consis{\qelem}$ but $\langle \qelem, v_{\pi}, \qelem', v_{\pi}, R\rangle\notin\rolesf$ for some $\qelem'\in\Delta$ with $(x'\col b)\in\consis{\qelem'}$. But by construction $v_{\pi}$ is in all elements in $\Delta$, hence there is at least one element such that $(v_{\pi}\col b)\in\consis{\qelem'}$, and since $\dlstruct,\pi\models R(a,b)$ then we have $(\qelem,\qelem')\in R^{\gamma(\pi)}$ and $\{\langle \qelem, v_{\pi}, \qelem', v_{\pi}, R\rangle\}\notin\rolesf$, thus the rule is not applicable.

                  \item $\mathbf{R}_{r'}$ is applicable if $\{v_{\pi} \col b,\ v_{\pi} \col R(a,b)\}\subseteq \consis{\qelem}$ but $\langle \qelem', v_{\pi}, \qelem, v_{\pi}, R\rangle\notin\rolesf$ for some $\qelem'\in\Delta$ with $(x'\col a)\in\consis{\qelem'}$. But by construction $v_{\pi}$ is in all elements in $\Delta$, hencec there is at least one element such that $(v_{\pi}\col a)\in\consis{\qelem'}$, and since $\dlstruct,\pi\models R(a,b)$ then we have $(\qelem',\qelem)\in R^{\gamma(\pi)}$ and $\{\langle \qelem', v_{\pi}, \qelem, v_{\pi}, R\rangle\}\notin\rolesf$, thus the rule is not applicable.

                  \item $\mathbf{R}_{\exists'}$ is applicable if there are some $\qelem,\qelem' \in\Delta$ with
                        $(v_{\pi} \col \exists R.C)\in \consis{\qelem}$,
                        $(C,\stlabel{\qelem}{v_{\pi}},x')\in\elabel{\qelem'}$ and $\qelem\neq\qelem'$ or $x=x'$ but $\langle \qelem, v_{\pi}, \qelem'', x'', R\rangle\notin\rolesf$ for all $\qelem'', x''$ with $(C,\stlabel{\qelem}{v_{\pi}},x'')\in\elabel{\qelem''}$ and $\qelem\neq\qelem''$ or $x=x''$. However, by construction we have $(v_{\pi} \col \exists R.C)\in \consis{\qelem}$ if $\qelem\in \exists R.C^{\gamma(\pi)}$, and thus there is some $\qelem''$ such that $(\qelem,\qelem'')\in R^{\gamma(\pi)}$ and $\qelem''\in C^{\gamma(\pi)}$. By construction it then follows that there is such $\langle \qelem, v_{\pi}, \qelem'',  v_{\pi}, R\rangle\in\rolesf$ with  $(C,\stlabel{\qelem}{v_{\pi}},v_{\pi})\in \elabel{\qelem''}$ and thus the rule is not applicable.

                  \item $\mathbf{R}_{\exists}$ is applicable if $(v_{\pi}\col \exists R.C)\in \consisu{\qelem}$ and there is no $\qelem'$ such that $(C,\stlabel{\qelem}{v_{\pi}},x)\in\elabel{\qelem'}$ and $\langle \qelem, v_{\pi}, \qelem', x', R\rangle\in\rolesf$ with $\qelem\neq\qelem'$ or $x=x'$. But by construction, if $(v_{\pi}\col \exists R.C)\in \consisu{\qelem}$ then $\qelem\in(\exists R.C)^{\gamma(\pi)}$ and thus there is some $\qelem'$ such that $(\qelem,\qelem')\in R^{\gamma(\pi)}$ and $\qelem'\in C^{\gamma(\pi)}$. Then, again by construction, $\consisu{\qelem'}$ has $(C, \stlabel{\qelem}{v_{\pi}},v_{\pi})\in\elabel{\qelem'}$ and $\langle \qelem, v_{\pi}, \qelem', v_{\pi}, R\rangle\in\rolesf$, thus the rule is not applicable.
              \end{itemize}
    \end{itemize}

    %%%%%%%% THE TUPLE IS A COMPLETION GRAPH
    To show that $\tuple{\Delta,\consisfu,\elabelf,\rolesf}$ is a completion graph, we must show that, by construction, for all $\langle \qelem, v, \qelem', v', R\rangle\in\rolesf$, $\qelem,\qelem'\in\Delta$ and $\stlabel{\qelem}{v}=\stlabel{\qelem'}{v'}$, which follows straightforwardly since $v=v'=v_{\pi}$ for some $\pi\in\Pi$ (first condition) and that if $(C,s,x_{\pi})\in\elabel{\qelem}$, then $\{(x\col C)\}\cup \{(x\col \st)\mid \st\in s\}\subseteq \consis{\qelem}$ (second condition).

    %%%%%%%% THE CG IS coherent
    We have thus shown that $\tuple{\Delta,\consisfu,\elabelf,\rolesf}$ is a completion graph for $\kb$ and that all of its constraint systems are globally complete and clash-free, then it remains to show that the constraint graph is coherent.
    Notice that since $\dlstruct$ is a model, there is a unique element $\qelem_a\in\Delta$ for each $a\in\objC$ by construction and such that $(v_{\pi}\col a)\in\consisu{\qelem_a}$ for all variables $v_{\pi}$ (first condition). Then, for all $\consis{\qelem}$ and $\consis{\qelem'}$, if $v_{\pi}$ is in $\consis{\qelem}$ it is also in $\consis{\qelem'}$ with $\stlabel{\qelem}{v_{\pi}}=\stlabel{\qelem'}{v_{\pi}}$ (second condition), and if $(v_{\pi}\col\phi)\in\consis{\qelem}$ then $\dlstruct,\pi\models\phi$, hence also $(v_{\pi}\col\phi)\in\consis{\qelem'}$ (third condition).% Finally, since $\tuple{\qelem, v_{\pi}, \qelem', v', R}\in\runsf$ only if $(\qelem,\qelem')\in R^{\gamma(\pi)}$ and $v_{\pi}=v'$, and $\qelem\in \exists R.C^{\gamma(\pi)}$ if $\qelem'\in C^{\gamma(\pi)}$ then we obtain that by construction $(r_{\pi}(\qelem)\col \exists R.C)\in\consis{\qelem}$ if $(r_{\pi}(\qelem')\col C)\in\consis{\qelem'}$ (fourth condition).

    %%%%%%%% GAMMA IS A SET OF RUNS
    Let us now show that $\runsf$ is a set of runs. First, recall that in every constraint system $\consisu{\qelem}$, each variable $v_{\pi}$ maps to a $\pi\in\Pi$ (including the variables $v_{\st}$) and that $\{v_{\pi}\col \st \mid \pi\in\sigma(\st)\}\subseteq \consisu{\qelem}$. It thus follows that if $r_{\pi}(\qelem) = v_{\pi}$ for all $\qelem\in\Delta$ and $(r_{\pi}(\qelem)\col \st)\in\consisu{\qelem}$, then $(r_{\pi}(\qelem')\col \st) \in \consisu{\qelem'}$ \ref{condition:run-standpoint}. %Moreover, if $(r_{\pi}(\qelem)\col \phi)\in\consisu{\qelem}$ then $\dlstruct, \pi \models \phi$, and hence $(r_{\pi}(\qelem')\col \phi) \in \consisu{\qelem'}$ for all $\qelem'\in\Delta$ \ref{condition:run-axiom}. 
    Then, by construction $\tuple{\qelem, v_{\pi}, \qelem', v', R}\in\runsf$ only if $(\qelem,\qelem')\in R^{\gamma(\pi)}$ and $v_{\pi}=v'$, and as usual for $r_{\pi}(\qelem)=v_{\pi}$ also $r_{\pi}(\qelem')=v_{\pi}$ \ref{condition:run-role}. Similarly, if $(r_{\pi}(\qelem)\col \exists R.C)\in\consis{\qelem}$ it is because $\qelem\in \exists R.C^{\gamma(\pi)}$, thus there is some $\qelem'$ such that $(\qelem,\qelem')\in R^{\gamma(\pi)}$ and $\qelem'\in C^{\gamma(\pi)}$. Consequently, by construction there is $(r_{\pi}(\qelem')\col C)\in\consisu{\qelem'}$ and $\tuple{\qelem, v_{\pi}, \qelem', v', R}\in\runsf$ \ref{condition:run-existential}.

    %%%%%%%% Q IS A QUASI-MODEL

    To finally show that $\mathcal{Q}$ is a quasi-model we notice that
    for every $\qelem\in\Delta$ and variable $v_{\pi}\in \stvar{\qelem}{*}$, there exists a run $r$ in $\runsf$ such that $r(\qelem)=v_{\pi}$, namely the run $r_{\pi}$

    ($\Leftarrow$) Suppose that $\kb$ is quasi-satisfied in the quasi-model $\mathcal{Q}=\tuple{\Delta,\consisfu,\elabelf,\rolesf, \runsf}$.
    Define a $\SEL$ structure $\dlstruct = \tuple{\Dom, \Precs, \sigma, \gamma}$ as follows:

    \begin{itemize}
        \item $\dlstruct$ uses the same domain $\Dom$ as $\mathcal{Q}$
        \item $\Pi = \runsf$, i.e. the set of precisifications of $\dlstruct$ coincides with the set of runs in $\mathcal{Q}$
        \item $\sigma(\st)=\{r \mid \qelem\in\Delta,\ (r(\qelem)\col \st)\in\consisu{\qelem}\}$
        \item $C^{\gamma(r)} = \{ \qelem\in\Delta \mid (r(\qelem)\col C)\in\consisu{\qelem}\}$ for all concept names $C$
        \item $R^{\gamma(r)} = \{(\qelem,\qelem')\mid \langle \qelem,r(\qelem),\qelem',r(\qelem'),R\rangle\in\rolesf\}$
        \item $a^{\gamma(r)} = \qelem_a$ for all $a\in\objC$
    \end{itemize}

    We claim that $\kb$ is satisfied in $\dlstruct$.
    Let us observe first that

    \begin{enumerate}
        \item for all $r\in\Pi$, $\qelem\in\Delta$ and $C\in\CC$ with $C$ of the form $D \sqcap E$ or $\exists R.D$, if $\qelem\in C^{\gamma(r)}$ then $(r(\qelem)\col C)\in \consisu{\qelem}$ (left hand side of axioms by the normal form)
              \begin{description}[leftmargin=0.3cm, itemindent=-0.1cm, itemsep=0.2cm]
                  \item[$(C=D \sqcap E)\ $] Suppose  $C=D \sqcap E$, so $\qelem\in (D\sqcap E)^{\gamma(r)}$. Then $\qelem\in D^{\gamma(r)}$ and $\qelem\in E^{\gamma(r)}$. Since $\dlstruct$ is defined such that $C^{\gamma(r)} = \{ \qelem\in\Delta \mid (r(\qelem)\col C)\in\consisu{\qelem}\}$ for all concept names $C$, it follows that $(r(\qelem)\col D) \in \consisu{\qelem}$ and $(r(\qelem)\col E) \in \consisu{\qelem}$. Finally, we obtain $(r(\qelem)\col D \sqcap E) \in \consisu{\qelem}$ as desired by the non-applicability of the $\mathbf{R}_{\sqcap}$ rule.
                  \item[$(C=\exists R.D)\ $]
                      Suppose $C=\exists R.D$, so $\qelem\in (\exists R.D)^{\gamma(r)}$.
                      Then we know that there exists $\qelem'\in\Delta$ such that  $(\qelem,\qelem')\in R^{\gamma(r)}$ and $\qelem'\in D^{\gamma(r)}$.
                      By the construction of $\dlstruct$, we set $\qelem'\in D^{\gamma(r)}$ if we have $(r(\qelem')\col D) \in\consisu{\qelem'}$, and we set $(\qelem,\qelem')\in R^{\gamma(r)}$ if $\langle \qelem,r(\qelem),\qelem',r(\qelem'),R\rangle\in\rolesf$.
                      From $\langle \qelem,r(\qelem),\qelem',r(\qelem'),R\rangle\in\rolesf$, $(r(\qelem')\col D) \in\consisu{\qelem'}$ and the non-applicability of the rule $\mathbf{R}_{\downarrow}$ we obtain $(r(\qelem)\col \exists R.D) \in\consisu{\qelem}$ as desired.
              \end{description}
        \item for all $r\in\Pi$, $\qelem\in\Delta$ and $C\in\CC$ with $C$ of the form $\exists R.D$, $\standbs D$ or $\standds D$, if $(r(\qelem)\col C)\in \consisu{\qelem}$  then  $\qelem\in C^{\gamma(r)}$ (right-hand side of axioms by the normal form)

              \begin{description}[leftmargin=0.3cm, itemindent=-0.1cm, itemsep=0.2cm]
                  \item[$(C=\exists R.D)\ $] Suppose  $C=\exists R.D$, so $(r(\qelem)\col \exists R.D) \in \consisu{\qelem}$. Then, by \Cref{def:run}.\ref{condition:run-existential} there is some $\qelem'\in\Delta$ such that $\langle \qelem,r(\qelem),\qelem',r(\qelem'),R\rangle\in\rolesf$ and $(r(\qelem')\col D)\in\consisu{\qelem'}$. Then by the construction of $\dlstruct$ it is the case that $(\qelem,\qelem')\in R^{\gamma(r)}$ and $\qelem'\in D^{\gamma(r)}$, and hence it follows that $\qelem\in (\exists R.D)^{\gamma(r)}$.

                  \item[$(C=\standds D)\ $] Now suppose $C=\standds D$, so $(r(\qelem)\col \standds D) \in \consisu{\qelem}$. Then, since $\consisu{\qelem}$ is a globally complete constraint system, we know that $(x'\col D)\in\consisu{\qelem}$ for some $x'\in \stvar{\qelem}{\st}$. And since $\mathcal{Q}$ is a quasi-model, there is a run $r'$ such that $r'(\qelem)=x'$, so we have that $(r'(\qelem)\col D)\in \consisu{\qelem}$ and $r'(\qelem)\in \stvar{\qelem}{\st}$. This implies (by the model construction) that $r'\in\stvar{S}{\st}$ and $\qelem\in (D)^{\gamma(r')}$, which in turn implies $\qelem\in (\standds D)^{\gamma(r)}$.

                  \item[$(C=\standbs D)\ $] Finally suppose $C=\standbs D$, so $(r(\qelem)\col \standbs D) \in \consisu{\qelem}$. Then, since $\consisu{\qelem}$ is a globally complete constraint system, we know that $(x'\col D)\in \consisu{\qelem}$ for all $x'\in \stvar{\qelem}{\st}$ (which is non-empty). Since $\mathcal{Q}$ is a quasi-model, for each $x'$ there is a run $r'$ such that $r'(\qelem)=x'$, so we have that $(r'(\qelem)\col D)\in \consisu{\qelem}$ and $r'(\qelem)\in \stvar{\qelem}{\st}$. This implies that $\qelem\in (D)^{\gamma(r')}$ for all
                      $r'\in\stvar{S}{\st}$, which in turn implies $\qelem\in (\standbs D)^{\gamma(r)}$.
              \end{description}

              Our last observation is that
        \item for all $r\in\Pi$, $\qelem\in\Delta$ and $\phi\in\forC$, if $(r(\qelem)\col \phi)\in \consisu{\qelem}$ then  $\dlstruct ,r\models\phi$


              This is proved by induction for all types of axioms allowed in the normal form. The base cases are:
              \begin{description}[leftmargin=0.3cm, itemindent=-0.1cm, itemsep=0.2cm]
                  \item[$\phi=C\sqsubseteq D\ $] Suppose $(r(\qelem)\col C\sqsubseteq D)\in \consisu{\qelem}$ and recall that in all $\qelem'\in\Delta$ there is also $(r(\qelem')\col C\sqsubseteq D)\in \consisu{\qelem'}$ (second condition of a run). Then, since the constraint systems are globally complete, for all $\qelem'\in\Delta$, if $(r(\qelem')\col C)\in \consisu{\qelem'}$ then $(r(\qelem')\col D)\in \consisu{\qelem'}$. By (1) if $\qelem'\in C^{\gamma(r)}$ then $(r(\qelem')\col C)\in \consisu{\qelem'}$ and by (2) if $(r(\qelem')\col D)\in \consisu{\qelem'}$ then $\qelem'\in C^{\gamma(r)}$ and $\qelem'\in D^{\gamma(r)}$, and hence $ C^{\gamma(r)}\subseteq D^{\gamma(r)}$.  It clearly follows that $\dlstruct, r \models C\sqsubseteq D$.
                  \item[$\phi=\st\preceq\sp\ $] Suppose $(r(\qelem)\col \st\preceq\st)\in \consisu{\qelem}$. Then, since $\consisu{\qelem}$ is globally complete, for all $r'(\qelem)\in\stvar{\qelem}{\st}$, then $r'(\qelem)\in\stvar{\qelem}{\sp}$. Recall that within a run $r'$ all variables have the standpoint constraints: if $(r(\qelem)\col \st)\in\consisu{\qelem}$, then $(r(\qelem')\col \st) \in \consisu{\qelem'}$  for all $\qelem,\qelem'\in\Delta$ and $\st\in\SC$. Then by construction, if $r'\in\sigma(\st)$ then $r'\in\sigma(\sp)$ and consequently $\dlstruct, r \models \st\preceq \sp$.
                  \item[$\phi=C(a)\ $] Suppose $(r(\qelem)\col C(a))\in \consisu{\qelem}$. Then since $\mathcal{Q}$ is a quasi-model and $a\in\objC$, there is a unique quasi-element $\qelem_a\in\Delta$ such that $(v\col a)\in\consisu{\qelem_a}$ for all variables $v$ in $\consisu{\qelem_a}$. Thus, $(r(\qelem_a)\col a)\in \consisu{\qelem_a}$ and since $r$ is a run then also $(r(\qelem_a)\col C(a))\in \consisu{\qelem_a}$ and since $\consisu{\qelem_a}$ is globally complete also $(r(\qelem_a)\col C)\in \consisu{\qelem_a}$. Consequently, $\qelem_a=a^{\gamma(r)}$ and $\qelem_a\in C^{\gamma(r)}$, thus $\dlstruct, r \models C(a)$.
                  \item[$\phi=R(a,b)\ $] Suppose $(r(\qelem)\col R(a,b))\in \consisu{\qelem}$. Then since $\mathcal{Q}$ is a quasi-model and $a,b\in\objC$, then there are two quasi-elements $\qelem_a, \qelem_b\in\Delta$ such that $(v\col a)\in\consisu{\qelem_a}$ and $(v\col b)\in\consisu{\qelem_b}$ for all variables in $\consisu{\qelem_a}$ and $\consisu{\qelem_b}$. Thus, $(r(\qelem_a)\col a)\in \consisu{\qelem_a}$, $(r(\qelem_b)\col b)\in \consisu{\qelem_b}$ and $(r(\qelem_a)\col R(a,b))\in \consisu{\qelem_a}$. Consequently, $\qelem_a=a^{\gamma(r)}$, $\qelem_b=b^{\gamma(r)}$ and $(\qelem_a,\qelem_b)\in R^{\gamma(r)}$, thus $\dlstruct, r \models R(a,b)$.
              \end{description}
              The only inductive step is
              \begin{description}[leftmargin=0.3cm, itemindent=-0.1cm, itemsep=0.2cm]
                  \item[$\phi=\standbs\psi\ $] Suppose $(r(\qelem)\col \standbs\psi)\in \consisu{\qelem}$. Then, since $\consisu{\qelem}$ is globally complete, $(r'(\qelem)\col \psi)\in \consisu{\qelem}$ for all $r'(\qelem)\in\stvar{\qelem}{\st}$. By the inductive hypothesis $\dlstruct, r' \models\psi$, and we note that $\sigma(\st)=\{r'\in R \mid \qelem\in\Delta, r'(\qelem)\in\stvar{\qelem}{\st}\}$. Therefore, $\dlstruct, r \models \standbs\psi$.
              \end{description}
    \end{enumerate}

    We conclude the proof by noticing that $(r(\qelem)\col \phi)\in \consisu{\qelem}$ for all $\phi\in\kb$, $\qelem\in\Delta$ and $r\in\runsf$ by \Cref{def:constraint-system} and the non-applicability of $\mathbf{R}_{\downarrow}$ rule. From this and the observation (3) we obtain that  $\dlstruct,r\models\phi$ and hence $\dlstruct$ is a model of $\kb$.

\end{proof}


\subsection{Termination and correctness}
\subsubsection{Termination}

\begin{lemma}\label{lemma:preceq-axioms-everywhere}
    Let $S$ be a constraint system for $\kb$ produced by the algorithm. Then $(\st\preceq\sp)\in\kb$ iff there is some $x$ such that $(x\col \st\preceq\sp)\in S$.
\end{lemma}

\begin{proof}
    ($\Rightarrow$) From the definition of a constraint system for $\kb$, for all $(\st\preceq\sp)\in\kb$ we have $(v_{*}\col \st\preceq\sp)\in S$. ($\Leftarrow$) It is easy to see from the tableau rules that $(x\col \st\preceq\sp)$ can only be introduced during the creation of $S$ or by copying a preexisting $(x'\col \st\preceq\sp)$ constraint in $S$. If $S$ is created during the initialisation of the algorithm, then $(x\col \st\preceq\sp)\in S$ because $(\st\preceq\sp)\in\kb$. Similarly, if $S$ is created by an $\mathbf{R}_{\exists}$ application, then  $(x\col \st\preceq\sp)\in\consis{\qelem_{\top}}$ and hence also $(\st\preceq\sp)\in\kb$.
\end{proof}

\def\initialcsll{S_{L}^{\kb}}
\def\initialcsc{S_{C}^{\kb}}

\begin{lemma}\label{lemma:same-standpoints}
    Let $S$ and $S'$ be locally complete constraint systems for $\kb$ produced by the algorithm.
    The set of `standpoint signatures' in $S$ and $S'$ is the same $\{ \stlabel{S}{v} \mid v \in\stvar{S}{*}\}=\{ \stlabel{S'}{v} \mid v \in\stvar{S'}{*}\}$ and its size is smaller or equal to the number of standpoints in $\kb$, i.e. $\card{\{ \stlabel{S}{v} \mid v \in\stvar{S}{*}\}} \leq \card{\SC}$.
\end{lemma}

\begin{proof}
    Let $\initialcsll$ be the constraint system obtained by exhaustively applying (only) the local labelling rules to $\initialcs$.
    It is clear that $\initialcsll$ has exactly $\card{\SC}$ variables and hence there are at most $\card{\SC}$ different standpoint signatures. We will prove the lemma by showing that for $S$ a constraint system for $\kb$ where no local rules are applicable, the set of standpoint labels in $S$ and $\initialcsll$ is the same.

    Upon observation of the tableau rules, we can see that for any variable $v$ in $S$ either
    \begin{description}
        \item{\bf Base Case:} $v$ is initialised with $\{(v\col \st),(v\col *) \}\subseteq  S$.
        \begin{enumerate}
            \item By the definition of $\initialcs$, there is a variable $v_{\st}$ in $\initialcs$ also initialised with $\{(v_{\st}\col \st),(v_{\st}\col *) \}\subseteq\initialcs$
            \item From Lemma \ref{lemma:preceq-axioms-everywhere} it follows that for some $x$ in $S$ and $x'$ in $S'$, we have $(x\col \sp\preceq\st)\in S$ iff $(x'\col \sp\preceq\st)\in S'$ iff $(\sp\preceq\st)\in\kb$.
            \item From the definition of a constraint system, if $(\sp\preceq\st)\in\kb$ then $(v_{*}\col \sp\preceq\st)$ in both $S$ and $S'$
            \item By the premise, the tableau rules, (2) and (3), if $(v\col \s{n})\in S$ and $\s{n}\notin\{\st, *\}$ then there is a chain $\{(v_{*}\col \s{0}\preceq\s{1}),\dots,(v_{*}\col \s{n-1}\preceq\s{n})\}\subseteq S$ with $\s{0}\in\{\st, *\}$ such that the respective $\mathbf{R}_{\preceq}$ rule applications introduced $(v\col \s{n})$ in $S$.
            \item By (2) and (4), also $\{(v_{*}\col \s{0}\preceq\s{1}),\dots,(v_{*}\col \s{n-1}\preceq\s{n})\}\subseteq S'$ such that the respective $\mathbf{R}_{\preceq}$ rule applications introduced $(v'\col \s{n})\in S'$.
            \item By (5) we obtain $\stlabel{S}{v}=\stlabel{\initialcsll}{v_{\st}}$ as desired.
        \end{enumerate}
        \item{\bf Inductive Step:} $v$ is initialised with $\{(v\col \st) \mid (v'\col \st)\in S', \st\in\SC \}$ for some $v'$ in $S'$.
        \begin{enumerate}
            \item By induction, we know that for $v'$ in $S'$ there is some $x$ in $\initialcs$ such that $\stlabel{S'}{v'}=\stlabel{\initialcsll}{x}$.
            \item By Lemma \ref{lemma:preceq-axioms-everywhere}, if $(x\col \st\preceq\sp)\in S$ for some $x$ in $S$ then $(\st\preceq\sp)\in\kb$ and then also $(x'\col \st\preceq\sp)\in S'$ for some variable $x'$ in $S'$.
            \item By (2), if $(v\col \sp)\in S$ then also $(v'\col \sp)\in S'$, and therefore  $\stlabel{S}{v}=\stlabel{S'}{v'}$.
            \item By (1) and (3) $\stlabel{S}{v}=\stlabel{\initialcsll}{x}$ as desired.
        \end{enumerate}
    \end{description}
\end{proof}

\begin{lemma}\label{lemma:num-elements-cs}
    Let $\mathbf{CG}$ be a completion graph for a knowledge base $\kb$ constructed by the algorithm. Then the number of elements in $\mathbf{CG}$ is bounded by $3\size{\kb}^2$.
\end{lemma}

\begin{proof}
    Let us first consider the number of elements in $\mathbf{CG}$ in its initialisation and then the number of new elements that can be produced by global rule applications. It is easy to see that during initialisation, we will produce exactly $1+\card{\objC}$ elements and $1+\card{\objC}\leq \size{\kb}$ (there is at least one formula in $\kb$). The applicability of the global generating rules depends on the preexistence of element labels of the form $(C,s,x)\in L$ that are different to the current node. Since global rules are only applicable to locally complete constraint systems (by the order imposed by the algorithm) and by Lemma \ref{lemma:same-standpoints} we know that there are at most $\card{\SC}$ different standpoint signatures in $\mathbf{CG}$ if it is locally consistent, then the rule $\mathbf{R}_{\exists}$ can produce at most $2\card{\SC}\times\card{\CC}\leq \size{\kb}^2$ different elements before no more rules are applicable in $\mathbf{CG}$.
\end{proof}

\begin{lemma}\label{lemma:num-constraints-per-element}
    Let $\mathbf{CG}$ be a completion graph for a knowledge base $\kb$ constructed by the algorithm and let $\qelem$ be an element in $\mathbf{CG}$. Then the number of variables in $\consis{\qelem}$ is bounded by $2\size{\kb}^2$ and the number of constraints in $\consis{\qelem}$ by $2\size{\kb}^3$
\end{lemma}

\begin{proof}
    Let us determine an upper bound for the number of distinct variables
    per element. First, an element produced during the initialisation of the tableau $\qelem_i\in\{\qelem_{\top}\}\cup\{\qelem_a\mid a\in\objC\}$ (its label, to be more precise) contains exactly $|\SC|$ distinct variables at the moment of its generation.% Since new marked variables are never produced, each element will always have at most $|\SC|$ marked variables.

    Consider now how can new %unmarked 
    variables be introduced in $\consis{\qelem_i}$. The only rule that locally introduces variables is $\mathbf{R}_{\Diamond}$, which applies to constraints of the form $\{x\col \standds C\}$. Notice that the normal form guarantees that any concept of the form $\standds C$ is the application of a modal operator to a basic concept $C\in\BCC$.
    There are at most $|\CC|$ different concepts of the form $\standds C$ and each can be applied at most once because the variable that triggers the rule does not play a role in its effect and no rule produces constraints of the form $x\col \standds C$ with $\standds C\notin \CC$. Therefore at most $|\CC|$ variables can be internally generated in $\consis{\qelem_i}$. Finally, the rules $\mathbf{R}_{r}$ and $\mathbf{R}_{r'}$ apply to named individuals and can introduce externally generated variables in $\consis{\qelem_i}$. Since there are at most $\size{\kb}$ elements for named individuals in $\mathbf{CG}$, each of which with $|\CC|$ internally generated variables, then $\size{\kb}^2$ variables can be externally introduced in $\consis{\qelem_i}$.

    Now, consider the elements that are generated via a global generating rule: Clearly, a new element $g$ produced by the $\mathbf{R}_{\exists}$ rule will have $\stvar{g}{*}=\stvar{\qelem_{\top}}{*}+1$ variables (notice that $\mathbf{R}_{r}$ and $\mathbf{R}_{r'}$ are never applicable to elements that are generated via a global generating rule).
    Since the variables from $\initialcs$ are copied to $g$ with their constraints, $g$ will still contain at most $|\CC|$ variables introduced by the $\mathbf{R}_{\Diamond}$ and an additional variable from the rule $\mathbf{R}_{\exists}$.

    Hence, we can conclude that every element $\qelem\in\mathbf{SC}$ has at most $2\size{\kb}^2$ variables. It should be clear that each variable can in turn be assigned to (a) each concept in $\CC$, (b) one individual in $\objC$, (c) each subformula in $\forC$ and (d) each standpoint in $\SC$, hence each variable has at most $\size{\kb}$ constraints. Consequently, there are at most $2\size{\kb}^3$ constraints in $\consis{\qelem}$.
\end{proof}

\begin{theorem}\label{theorem:termination}
    The completion algorithm terminates after at most $c\size{\kb}^6$ steps, where $c$ is a constant.
\end{theorem}

\begin{proof}
    In view of Lemma \ref{lemma:num-elements-cs}, there are at most $3\size{\kb}^2$ elements in each completion graph constructed by the algorithm. As every global generating rule adds a new node, the number of applications of such rules ($\mathbf{R}_{\exists}$) is bounded by the same number.

    Now let us compute the number of applications of the rest of tableau rules. Since the rules $\mathbf{R}_{\preceq}$, $\mathbf{R}_{\sqcap}$, $\mathbf{R}_{\sqsubseteq}$, $\mathbf{R}_{\Box}$, $\mathbf{R}_{\Diamond}$, $\mathbf{R}_{g}$,
    $\mathbf{R}_{a}$, $\mathbf{R}_{r}$, $\mathbf{R}_{r'}$ and $\mathbf{R}_{\downarrow}$ produce one or more new constraints in an element, and from Lemma \ref{lemma:num-constraints-per-element} we know that there are at most $2\size{\kb}^3$ constraints in every element, then the number of applications of such rules per element is bounded by the same number.

    The only rule that does not produce new constraints is $\mathbf{R}_{\exists'}$. This rule can add, for each $\qelem$ with $(C,s,x)\in\elabel{\qelem}$, at most one quasi-role from every variable in every element. Recall that by the rules of the algorithm, no element is generated with more than one label. Since the bound on variables per object is $2\size{\kb}^2$ and the bound in the size of the domain is $3\size{\kb}^2$, then we have at most $6\size{\kb}^4$ rule applications.

    Finally, the number of applications of these rules during the execution of the algorithm is bounded by the bound on rule applications per element multiplied by the bound on elements, and together with the bound on $\mathbf{R}_{\exists}$ that gives us the total bound on tableau rule applications:
    $$ (6\size{\kb}^4)(3\size{\kb}^2) + (2\size{\kb}^3)(3\size{\kb}^2) + 3\size{\kb}^2 \leq (27\size{\kb}^6) $$

\end{proof}

\subsubsection{Soundness and Completeness}
\begin{theorem}[Soundness]\label{theorem:soundness}
    If there is a globally complete, coherent and clash-free completion graph $\mathbf{CG}$ for a knowledge base $\kb$, then $\kb$ is satisfiable.
\end{theorem}

\begin{proof}
    We will show that if there is a globally complete, coherent and clash-free completion graph $\mathbf{CG}$ for a $\SEL$ knowledge base $\kb$, then there is a quasi-model for $\kb$. If there is a quasi-model for $\kb$ it follows that $\kb$ is quasi-satisfiable, and by Theorem \ref{theorem:satisfiable-iff-quasisatisfiable}, if $\kb$ is quasi-satisfiable then it is satisfiable.

    Let $\mathbf{CG}=\tuple{\Delta,\consisf,\elabelf,\rolesf}$ be a globally complete, coherent and clash-free completion graph for $\kb$. Set $\mathcal{Q}=\tuple{\Delta,\consisf,\elabelf,\rolesf,\runsf}$, where $\runsf$ are all possible runs %and $\rolesf$ are all possible quasi-roles 
    on $\mathcal{Q}$. To show that $\mathcal{Q}$ is a quasi-model for $\kb$, we show that we can generate a run in $\mathcal{Q}$ with $r(\qelem)=v$ for each variable  $v$ in $\consisu{\qelem}$, with $\qelem\in\Delta$.
    \begin{description}
        \item[\ref{condition:run-standpoint}:] By \Cref{def:coherence} we have that if $r(\qelem)=v$, then for each $\qelem'\in\Delta$ there is some $v'$ such that $\stlabel{\qelem}{v}=\stlabel{\qelem'}{v'}$ such that we can set $r(\qelem')=v'$.
        \item [\ref{condition:run-role}:] Moreover, from the definition of a constraint graph we know that if $\tuple{\qelem', v', \qelem, v, R}\in\rolesf$ then $\stlabel{\qelem}{v}=\stlabel{\qelem'}{v'}$. Then, by the non-applicability of the $\mathbf{R}_{\downarrow}$ rule, we have that $(v' \col \exists R.C) \in\consisu{\qelem}$ if $(v\col C)\in\consisu{\qelem'}$. Thus, we can generate a run with $r(\qelem)=v$ and $r(\qelem')=v'$ also satisfying \ref{condition:run-standpoint}.
        \item [\ref{condition:run-existential}:] If $(v\col \exists R.C) \in\consisu{\qelem}$, then from the non-applicability of $\mathbf{R}_{\exists}$ there must be some $\qelem'\neq\qelem$ such that $(C,s,x)\in\elabel{\qelem'}$, $s=\stlabel{\qelem}{v}$ and $\tuple{\qelem, r(\qelem), \qelem', x, R}\in\rolesf$. It is clear that we can generate a run with $r(\qelem)=v$ and $r(\qelem')=v'$ also satisfying \ref{condition:run-standpoint} and \ref{condition:run-role}.
    \end{description}
    Hence we conclude that $\mathcal{Q}$ is a quasi-model for $\kb$.
\end{proof}

\begin{lemma}\label{lemma:same-axiom-per-standpoint}
    Let $\mathbf{CG}$ be a locally complete completion graph for $\kb$ produced by the algorithm, and let $\qelem, \qelem'$ be elements of $\mathbf{CG}$. For all variables $v$ in $\consis{\qelem}$ and $v'$ in $\consis{\qelem'}$ it is the case that if $\stlabel{{\qelem}}{v}=\stlabel{{\qelem'}}{v'}$ then $\{\phi \mid (v\col \phi)\in\consis{\qelem}\}=\{\phi\mid(v'\col \phi)\in\consis{\qelem'}\}$.
\end{lemma}

\begin{proof}

    We show that if $\stlabel{{\qelem}}{v}=\stlabel{{\qelem'}}{v'}$ and $(v\col \phi)\in\consis{\qelem}$ then $(v'\col \phi)\in\consis{\qelem'}$.

    \noindent If $(v\col \phi)\in\consis{\qelem}$ then clearly either (1) $\phi\in\kb$ or (2) $\phi\in\forC$.
    \begin{enumerate}
        \item If $(v\col \phi)\in\consis{\qelem}$ and $\phi\in\kb$. By the definition of a constraint system for $\kb$ we have $(v_*\col \phi)\in\consis{\qelem'}$, and since the normal form forces all axioms in $\kb$ to be of the form $\st\preceq\sp$ or $\standbs\psi$, we obtain $(v'\col \phi)\in\consis{\qelem'}$ from the non-applicability of $\mathbf{R}_{g}$.

        \item If $(v\col \phi)\in\consis{\qelem}$ and $\phi\in\forC$ but $\phi\notin\kb$
              \begin{enumerate}
                  \item It can only be that there is a formula $\standbs\phi\in\kb$
                  \item Notice that given (2) and (a), the constraint $(v\col \phi)\in\consis{\qelem}$ can only have been produced by a rule $\mathbf{R}_{\Box}$ or $\mathbf{R}_{\exists}$. We show that $\{(v\col \standbs\phi),(v\col \st)\}\subseteq\consis{\qelem}$:
                        \begin{description}
                            \item [Case 1:] $(v\col \phi)\in\consis{\qelem}$ was produced by $\mathbf{R}_{\Box}$. Then by the conditions of the rule $\{(v\col \standbs\phi),(v\col \st)\}\subseteq\consis{\qelem}$
                            \item [Case 2:] $(v\col \phi)\in\consis{\qelem}$ was produced by $\mathbf{R}_{\exists}$. Then $(v\col \phi)\in\consis{\qelem_{\top}}$. Then by \emph{Case 1} on $\qelem_{\top}$ we have $\{(v\col \standbs\phi),(v\col \st)\}\subseteq\consis{\qelem_{\top}}$ and by the same $\mathbf{R}_{\exists}$ rule also  $\{(v\col \standbs\phi),(v\col \st)\}\subseteq\consis{\qelem}$
                        \end{description}
                  \item By (b) and the non-applicability of the rule  $\mathbf{R}_{\Box}$ we have $(v'\col \phi)\in\consis{\qelem'}$ as desired.
              \end{enumerate}
    \end{enumerate}

\end{proof}
% \iffalse
% \begin{lemma}\label{lemma:some-marked-var}
%     Let $\mathbf{CG}$ be a globally complete completion graph for $\kb$ produced by the algorithm and $S$ a constraint system in $\mathbf{CG}$. For all $v$ in $S$ there is some $v_{\st}$ in $S$ such that $\stlabel{S}{v}=\stlabel{S}{v_{\st}}$, $v_{\st}$ is also in $\initialcs$ and for $\mathds{C}$ a concept $C\in\CC$, an individual $a\in\objC$ or a subformula $\phi\in\forC$, then if $(v_{\st}\col \mathds{C})\in S$, then $(v\col \mathds{C})\in S$.
% \end{lemma}

% \begin{proof}
%     Let $\initialcsll$ be the constraint system obtained by exhaustively applying (only) the local labelling rules to $\initialcs$. Notice that $\initialcs\subseteq\initialcsll\subseteq S$. Upon observation of the tableau rules, we can see that for any variable $v$ in $S$ either
%      \begin{description}
%         \item{\bf Base Case:} $v$ is initialised with $\{(v\col \st),(v\col *),(v\col \top) \}\subseteq  S$ (it is possible that $\st = *$). 
%         %\begin{enumerate}
%             By the definition of $\initialcs$, there is a variable $v_{\st}$ in $\initialcs$  initialised with $\{(v_{\st}\col \st),(v_{\st}\col *),(v_{\st}\col \top), (v_{\st}\col \phi)\mid \phi\in\kb \}\subseteq\initialcs$.
%             Moreover, from the non-applicability of the rule $\mathbf{R}_{g}$ (\Cref{fig:rules}), it is clear that $\{(v\col \phi)\mid \phi\in\kb \}\subseteq S$. 
%             From the rest of tableau rules (\Cref{fig:rules}), if a rule is applicable to $v_{\st}$, then it is also applicable to $v$. Hence, if a constraint $(v_{\st}\col \st)$ or $(v_{\st}\col C)$ is added to $S$ after a sequence of rule applications, then a constraint $(v\col C)$ has also been added to $S$. %Notice that the global rules $\mathbf{R}_{\downarrow}$ and $\mathbf{R}_{r}$ can introduce constraints on $v_{\st}$ with $S$ remaining locally complete. Those constraints however do not lead to the introduction of any constraints of the form $(v_{\st}\col \st)$ or $(v_{\st}\col C)$ and are thus harmless for the local claim. When $S$ is globally complete, then it is clear that if a constraint $(v_{\st}\col \mathds{C})$ is added to $S$ after a sequence of local rule applications, then a constraint $(v\col \mathds{C})$ has also been added to $S$.
%         %\end{enumerate}
%         \item{\bf Inductive Step:} $v$ is initialised with $\{(v\col \st) \mid (v'\col \st)\in S', \st\in\SC \}$ for some $v'$ in $S'$. 
%         %\begin{enumerate}
%          By Lemma \ref{lemma:same-standpoints}, we know that for $v'$ in $S'$ there is some $v_{\st}$ in $\initialcs$ such that $\stlabel{S'}{v'}=\stlabel{\initialcsll}{v_{\st}}$. And since $\initialcsll\subseteq S$, then $\stlabel{S}{v}=\stlabel{S}{v_{\st}}$. Like before, by the non-applicability of the rule $\mathbf{R}_{g}$ we have again $\{(v\col \phi)\mid \phi\in\kb \}\subseteq S$, and through the same reasoning as before the lemma is proved.
%         %\end{enumerate}
%     \end{description}
% \end{proof}
% \fi

\begin{theorem}[Completness]
    If a $\SEL$ knowledge base $\kb$ is satisfiable, then %there is a complete and clash-free completion graph $\mathbf{CG}$ for $\kb$.
    %having started from $\qelemg_{\top}$, 
    the satisfiability-checking algorithm for $\SEL$ will construct a globally complete, coherent and clash-free completion graph for $\kb$.
\end{theorem}
\begin{proof}
    If $\kb$ is satisfiable then it is quasi-satisfiable (Theorem \ref{theorem:satisfiable-iff-quasisatisfiable}), and hence there is a quasi-model $\mathcal{Q}=\tuple{\Delta^q,\consisfq,\elabelf^q,\rolesf^q,\runsf^q}$ for $\kb$. We use $\mathcal{Q}$ as a guide and the tableau rules to construct a globally complete, coherent and clash-free completion tree $\mathbf{CG}=\tuple{\Delta,\consisf,\elabelf,\rolesf}$ for $\kb$. For the sake of better readability, let us  refer to the elements of $\Delta$ with $\qelemg, \qelemg', \dots$ and to the elements of $\Delta^q$ with $\qelem, \qelem', \dots$.

    Say that a completion graph $\mathbf{CG}$ for $\kb$ is $\mathcal{Q}$-compatible if the following holds:
    \begin{itemize}[label={-}]
        \item There is a relation $\mu \subseteq \Delta\times\Delta^q$ such that, for all $\qelemg\in\Delta$ and $\qelem\in\Delta^{q}$, $(\qelemg,\qelem)\in\crel$ if:
              \begin{itemize}
                  \item if $(x\col a)\in\consis{\qelemg}$ then $(v\col a)\in\consisq{\qelem}$ for every individual $a\in\objC$ and
                  \item $\elabel{\qelemg}\subseteq\elabelq{\qelem}$.
              \end{itemize}
        \item For each $\qelemg\in\Delta$ there is at least one pair $(\qelemg,\qelem)\in\crel$.
              %\item We use $\mu$ from the set of elements in $\Delta$ to $\Delta^q$
        \item For each pair $(\qelemg,\qelem)$ in $\crel$, there is a (total) surjective function $\cfuncf{\qelemg,\qelem}$ from the set of variables in $\consisq{\qelem}$ to the set of variables in $\consis{\qelemg}$ such that for $\cfunc{\qelemg,\qelem}{v}=x$
              \begin{itemize}
                  %  \item $\stlabel{\qelemg}{x}\subseteq\stlabel{\qelem}{v}$ and
                  \item  if $(x\col \st)\in\consis{\qelemg}$ then $(v\col \st)\in\consisq{\qelem}$ and
                  \item  if $(x\col \Phi)\in\consis{\qelemg}$ then $(v\col \Phi)\in\consisq{\qelem}$.
              \end{itemize}
        \item If $\tuple{\qelemg, x, \qelemg', x', R}\in\rolesf$, then there are some $(\qelemg,\qelem), (\qelemg',\qelem')\in\crel$ with $\cfunc{\qelemg,\qelem}{y}=x$ and $\cfunc{\qelemg',\qelem'}{y'}=x'$ and $\tuple{\qelem, y, \qelem', y', R}\in\rolesf^q$
    \end{itemize}


    \begin{claim}
        The completion graph $\mathbf{CG}_{\kb}=\tuple{\Delta,\consisf,\elabelf,\rolesf}$ for $\kb$ with
        \begin{itemize}
            \item $\Delta=\{\qelemg_{\top}\}\cup\{\qelemg_{a}\mid a\in\objC\}$,
            \item $\consis{\qelemg_{\top}}=\initialcs$ and $\elabel{\qelemg_{\top}}=\emptyset$,
            \item $\consis{\qelemg_{a}}=\initialcs \cup \{(x_{\st}\col a)\mid x_{\st}\in\stvar{\initialcs}{*} \}$ and $\elabel{\qelemg_{a}}=\emptyset$ for each $a\in\objC$, and
            \item $\rolesf=\emptyset$
        \end{itemize}
        is $\mathcal{Q}$-compatible.
    \end{claim}

    Recall that $\initialcs= \{(x_{\st}\col *), (x_{\st}\col \top), (x_{\st}\col \phi),  (x_{\st}\col \st) \mid \phi\in\kb, \st\in\SC \}$. By the definition of a completion graph, $\Delta^q$ is non-empty. It is clear that for all elements $\qelem\in\Delta^q$ we have $(\qelemg_{\top},\qelem)\in\crel$. Moreover, by the definition of a quasi-model, for each $a\in\objC$ there is a unique quasi-element $\qelem_a\in\Delta^q$ such that $(v\col a)\in\consisq{\qelem_a}$ for all variables $v$ in $\consisq{\qelem_a}$. Set $(\qelemg_a,\qelem_a)\in\crel$. From the former and the fact that for all $\qelemg\in\Delta$ we have $\elabel{\qelemg}=\emptyset$, it is clear that $\crel$ is as required. Notice that by definition $\initialcs\subseteq\elabelq{\qelem}$ for all $\qelem\in\Delta^q$ and if $(x\col a)\in\consis{\qelemg_a}$ then also $(v\col a)\in\consisq{\qelem_a}$. Then we can set $\cfunc{\qelemg,\qelem}{v_{\st}}=x_{\st}$ for each $(\qelemg,\qelem)\in\crel$, $x_{\st}$ in $\consis{\qelemg}$ and $v_{\st}$ in $\qelem$. Moreover, for $v$ in $\qelem$ there is some $v_{\st}$ such that $\stlabel{\qelem}{v}=\stlabel{\qelem}{v_{\st}}$, thus we can set $\cfunc{\qelemg,\qelem}{v}=\cfunc{\qelemg,\qelem}{v_{\st}}$. It should be clear that $\cfuncf{\qelemg,\qelem}$ is as required.

    \begin{claim}
        If a completion graph $\mathbf{CG}$ for $\kb$ is $\mathcal{Q}$-compatible and $\mathbf{CG}'$ is the result of an application of a rule $\mathbf{R}$ to $\mathbf{CG}$, then $\mathbf{CG}'$ is $\mathcal{Q}$-compatible as well.
    \end{claim}

    Let $\mathbf{CG}$ be an $\mathcal{Q}$-compatible completion graph, $\qelemg$ an element in $\mathbf{CG}$ and let $\crel$ and for all $(g,\qelem)\in\crel$ let $\cfuncf{\qelemg,\qelem}$ be the functions supplied by the definition of $\mathcal{Q}$-compatibility. Let us consider all the cases for $\mathbf{R}$.

    \begin{description}[itemsep=0.2cm]
        \item[$\mathbf{R}_{\preceq}\ $] Suppose that the rule $\mathbf{R}_{\preceq}$ is applicable to the constraints $\{(x\col \st\preceq \sp), (x'\col \st)\}\subseteq\consis{\qelemg}$ with $(x'\col \sp)\notin\consis{\qelemg}$. Let $(\qelemg,\qelem)\in\crel$ and $y$ and $y'$ be variables in $\consisq{\qelem}$ such that $\cfunc{\qelemg,\qelem}{y} = x$ and $\cfunc{\qelemg,\qelem}{y'} = x'$. Then we have $\{(y\col \st\preceq \sp),(y'\col \st)\}\subseteq\consisq{\qelem}$. The non-applicability of $\mathbf{R}_{\preceq}$ to $\consisq{\qelem}$ means that $(y' \col \sp) \in \consisq{\qelem}$. The application of the $\mathbf{R}_{\preceq}$ rule adds $(x' \col \sp) \in \consis{\qelemg}$. Hence, the relation $\crel$ and the function $\cfuncf{\qelemg,\qelem}$ are as required for the resulting completion graph $\mathbf{CG}'$.

        \item[$\mathbf{R}_{\sqcap}\ $] Suppose that the rule $\mathbf{R}_{\sqcap}$ is applicable to the constraints $\{x \col C, x\col D\} \subseteq\consis{\qelemg}$. Let $(\qelemg,\qelem)\in\crel$ and $y$ be a variable in $\consisq{\qelem}$ such that  $\cfunc{\qelemg,\qelem}{y} = x$. Then we have $\{y \col C, y\col D\} \subseteq \consisq{\qelem}$. The non-applicability of $\mathbf{R}_{\sqcap}$ to $\consisq{\qelem}$ means that $(y \col C \sqcap D) \in \consisq{\qelem}$. The application of the $\mathbf{R}_{\sqcap}$ rule adds $(x \col C \sqcap D) $ to $\consis{\qelemg}$. Hence, the relation $\crel$ and the function $\cfuncf{\qelemg,\qelem}$ are as required for the resulting completion graph $\mathbf{CG}'$.

        \item[$\mathbf{R}_{\sqsubseteq}\ $] Suppose that the rule $\mathbf{R}_{\sqsubseteq}$ is applicable to the constraints $\{x\col C, x\col C\sqsubseteq D\} \subseteq\consis{\qelemg}$. Let $(\qelemg,\qelem)\in\crel$ and $y$ be a variable in $\consisq{\qelem}$ such that $\cfunc{\qelemg,\qelem}{y} = x$. Then we have $\{y \col C, y\col C\sqsubseteq D\} \subseteq \consisq{\qelem}$. The non-applicability of $\mathbf{R}_{\sqsubseteq}$ to $\consisq{\qelem}$ means that $(y \col D) \in \consisq{\qelem}$. The application of the $\mathbf{R}_{\sqsubseteq}$ rule adds $(x \col D) $ to $\consis{\qelemg}$. Hence, the relation $\crel$ and the function $\cfuncf{\qelemg,\qelem}$ are as required for the resulting completion graph $\mathbf{CG}'$.

        \item[$\mathbf{R}_{\Box}\ $] Suppose that the rule $\mathbf{R}_{\Box}$ is applicable to the constraints $\{x\col \standbs \Phi, x'\col \st\}\subseteq\consis{\qelemg}$ with $(x \col \Phi)\notin\consis{\qelemg}$. Let $(\qelemg,\qelem)\in\crel$ and $y$ and $y'$ be variables in $\consisq{\qelem}$ such that $\cfunc{\qelemg,\qelem}{y} = x$ and $\cfunc{\qelemg,\qelem}{y'} = x'$. Then we have $\{y\col \standbs \Phi,\ y'\col \st\}\subseteq\consisq{\qelem}$. The non-applicability of $\mathbf{R}_{\Box}$ to $\consisq{\qelem}$ means that $(y' \col \Phi) \in \consisq{\qelem}$. The application of the $\mathbf{R}_{\Box}$ rule adds $(x' \col \Phi) $ to $\consis{\qelemg}$. Hence, the relation $\crel$ and the function $\cfuncf{\qelemg,\qelem}$ are as required for the resulting completion graph $\mathbf{CG}'$.

        \item[$\mathbf{R}_{g}\ $] Suppose that the rule $\mathbf{R}_{g}$ is applicable to the constraint $\{x \col \mathbf{G}\}\subseteq\consis{\qelemg}$ with $(x' \col \mathbf{G})\notin\consis{\qelemg}$ for some $x'$ in $\consis{\qelemg}$. Let $(\qelemg,\qelem)\in\crel$ and $y$ and $y'$ be variables in $\consisq{\qelem}$ such that $\cfunc{\qelemg,\qelem}{y} = x$ and $\cfunc{\qelemg,\qelem}{y'} = x'$. Then we have $\{y\col \mathbf{G}\} \subseteq \consisq{\qelem}$. The non-applicability of $\mathbf{R}_{g}$ to $\consisq{\qelem}$ means that $(y' \col \mathbf{G}) \in \consisq{\qelem}$. The application of the $\mathbf{R}_{g}$ rule adds $(x' \col \mathbf{G}) $ to $\consis{\qelemg}$. Hence, the relation $\crel$ and the function $\cfuncf{\qelemg,\qelem}$ are as required for the resulting completion graph $\mathbf{CG}'$.

        \item[$\mathbf{R}_{a}\ $] Suppose that the rule $\mathbf{R}_{a}$ is applicable to the constraints $\{x\col a, x\col C(a)\} \subseteq\consis{\qelemg}$. Let $(\qelemg,\qelem)\in\crel$ and $y$ be a variable in $\consisq{\qelem}$ such that $\cfunc{\qelemg,\qelem}{y} = x$. Then we have $\{y \col a, y\col C(a)\} \subseteq \consisq{\qelem}$. The non-applicability of $\mathbf{R}_{a}$ to $\consisq{\qelem}$ means that $(y \col C) \in \consisq{\qelem}$. The application of the $\mathbf{R}_{a}$ rule adds $(x \col C) $ to $\consis{\qelemg}$. Hence, the relation $\crel$ and the function $\cfuncf{\qelemg,\qelem}$ are as required for the resulting completion graph $\mathbf{CG}'$.

        \item[$\mathbf{R}_{\Diamond}\ $] Suppose that the rule $\mathbf{R}_{\Diamond}$ is applicable to the constraint $(x\col \standds C)\in\consis{\qelemg}$ with no $x'$ in $\consis{\qelemg}$ such that $\{x' \col \st,\ x' \col C\}\subseteq \consis{\qelemg}$. Let $(\qelemg,\qelem)\in\crel$ and $y$ be a variable in $\consisq{\qelem}$ such that $\cfunc{\qelemg,\qelem}{y} = x$. Then we have $(y\col \standds C)\in\consisq{\qelem}$. The non-applicability of $\mathbf{R}_{\Diamond}$ to $\consisq{\qelem}$ means that there exists $y'$ in $\consisq{\qelem}$ such that $\{y' \col \st,\ y' \col C\}\subseteq\consisq{\qelem}$. The application of the $\mathbf{R}_{\Diamond}$ rule to $\consis{\qelemg}$ creates a fresh variable $x'$  and sets $\{x' \col \st,\ x' \col C\}\subseteq \consis{\qelemg}$. Then we define $\cfuncfp{\qelemg,\qelem}$ as the update of $\cfuncf{\qelemg,\qelem}$ with $\cfuncp{\qelemg,\qelem}{y'} = x'$ (notice that  if $(x'\col \st)\in\consis{\qelemg}$ then $(y'\col \st)\in\consisq{\qelem}$). Hence, the relation $\crel$ and the function $\cfuncfp{\qelemg,\qelem}$ are as required for the resulting completion graph $\mathbf{CG}'$.

        \item[$\mathbf{R}_{\exists}\ $] Suppose that the rule $\mathbf{R}_{\exists}$ is applicable to the constraint $(x\col \exists R.C) \in\consis{\qelemg}$ since there is no $\qelemg'\in\Delta$ such that $(C,\stlabel{\qelemg}{x},x')\in\elabel{\qelemg'}$, $\langle \qelemg, x, \qelemg', x', R\rangle\in\rolesf$ and $\qelemg'\neq \qelemg$. Let $(\qelemg,\qelem)\in\crel$ and $y$ be a variable in $\consisq{\qelem}$ such that $\cfunc{\qelemg,\qelem}{y} = x$. Then we have $(y\col \exists R.C) \in\consisq{\qelem}$. The non-applicability of $\mathbf{R}_{\exists}$ to $\consisq{\qelem}$ means that there exists $\qelem^q$ in $\Delta^q$ such that $(C,s,y')\in\elabelq{\qelem^q}$ with $s=\stlabel{\qelem}{y}$ and $\langle \qelem, y, \qelem', y', R\rangle\in\rolesf$. This implies that $\{y'\col C,\ y'\col \top\}\cup\{y'\col \st \mid (y\col \st)\in\consisq{\qelem}, \st\in\SC \}\subseteq\consisq{\qelem^q}$. The rule application of $\mathbf{R}_{\exists}$ to $\consis{\qelemg}$ generates an element $\qelemg'$ with $\elabel{\qelemg'}=(C,\stlabel{\qelemg}{x},x')$, $\rolesf:=\rolesf\cup \{\langle \qelemg, x, \qelemg', x', R\rangle\}$ and $\consis{\qelemg'}=\consis{\qelemg_{\top}}\cup\{x'\col C,\ x'\col \top\}\cup\{x'\col \st \mid (x\col \st)\in\consis{\qelemg}, \st\in\SC \}$. We define $\crel'$ as the extension of $\crel$ such that $(\qelemg',\qelem')\in\crel'$ for all $\qelem'\in\Delta^q$ with $(C,s,y')\in\elabelq{\qelem'}$. Note that there is at least one element, $\qelem^q$, such that $(\qelemg',\qelem^q)\in\crel'$.

            Now, we must define $\cfuncf{\qelemg',\qelem'}$ for each $(\qelemg',\qelem')\in\crel'$. It is clear that we can set $\cfunc{\qelemg',\qelem'}{y'}=x'$. For the rest of variables $x_{\st}\in\stvar{\qelemg'}{*}$ such that $x_{\st}\neq x'$, we recall that $\initialcs= \{(x_{\st}\col *), (x_{\st}\col \top), (x_{\st}\col \phi),  (x_{\st}\col \st) \mid \phi\in\kb, \st\in\SC \}$ and that by the definition of a constraint system $\initialcs\subseteq\consisq{\qelem'}$. Then, we can set $\cfunc{\qelemg',\qelem'}{y_{\st}}=x_{\st}$ for each $x_{\st}\in\stvar{\qelemg'}{*}$ with $y_{\st}$ in $\consisq{\qelem^q}$ and for every unassigned $y''$ in $\consisq{\qelem^q}$ there is some $y_{\st}$ such that $\stlabel{\qelem^q}{y''}=\stlabel{\qelem^q}{y_{\st}}$ (by \Cref{def:coherence}) and thus we set $\cfunc{\qelemg',\qelem'}{y''}=x_{\st}$.

            Again, $\crel'$ and each $\cfuncf{\qelemg',\qelem'}$ is as required for the resulting completion graph $\mathbf{CG}'$:
            \begin{itemize}[label={-}]
                \item $\elabel{\qelemg'}\subseteq\elabelq{\qelem'}$,
                \item  for $x\in\stvar{\qelemg'}{*}$ and $\cfunc{\qelemg',\qelem'}{y}=x$, if $(x\col \st)\in\consis{\qelemg'}$ then $(y\col \st)\in\consisq{\qelem'}$,
                \item  for $x\in\stvar{\qelemg'}{*}$ and $\cfunc{\qelemg',\qelem'}{y}=x$, if $(x\col \Phi)\in\consis{\qelemg'}$ then $(y\col \Phi)\in\consisq{\qelem'}$,
                \item  for $\langle \qelemg, x, \qelemg', x', R\rangle\in\rolesf$ we have $\langle \qelem, y, \qelem^q, y', R\rangle\in\rolesf^q$ with $\cfunc{\qelemg',\qelem^q}{y'}=x'$
            \end{itemize}

        \item[$\mathbf{R}_{\downarrow}\ $]
            Suppose that the rule $\mathbf{R}_{\downarrow}$ is applicable since $(x\col C)\in \consis{\qelemg}$ and $\langle \qelemg', x', \qelemg, x, R\rangle\in\rolesf$, but $(x' \col \exists R.C)\notin \consis{\qelemg'}$.

            %    First, notice that, since $\mathbf{CG}$ is produced by the tableau algorithm, there is at most one element $\qelemg'\in\Delta$ with $\elabel{\qelemg'}=\{(C,\stlabel{\qelemg}{x},x')\}$ (see the tableau rules \Cref{fig:rules}). Moreover, by the construction of $\crel$ (notably by the rule $\mathbf{R}_{\exists}$) for all $\qelem'\in\Delta^q$ such that $(C,s,y')\in\elabelq{\qelem'}$ we have $(\qelemg',\qelem')\in\crel'$. Let $\upepsilon_{\qelemg'}=\{\qelem'\mid(\qelemg',\qelem')\in\crel'\}$.

            Let $(\qelemg,\qelem),(\qelemg',\qelem')\in\crel$, $y$ be a variable in $\consisq{\qelem}$ such that $\cfunc{\qelemg,\qelem}{y} = x$ and $y'$ a variable in $\consisq{\qelem'}$ such that $\cfunc{\qelemg',\qelem'}{y'} = x'$. Then we have $(y\col C) \in\consisq{\qelem}$ and $\langle \qelem', y', \qelem, y, R\rangle\in\rolesf^q$. By the non-applicability of the $\mathbf{R}_{\downarrow}$ rule on $\mathcal{Q}$ we have that $(y'\col \exists R.C)\in\consisq{\qelem'}$

            On the other hand, the application of the rule $\mathbf{R}_{\downarrow}$ adds $(x \col \exists R.D)$ to $\consis{\qelemg}$. Consequently, the relation $\crel$ and the functions $\cfuncf{\qelemg,\qelem}$ and $\cfuncf{\qelemg',\qelem'}$ are as required for the resulting completion graph $\mathbf{CG}'$.

        \item[$\mathbf{R}_{r}\ $]
            Suppose that the rule $\mathbf{R}_{r}$ is applicable to the constraints $\{x \col a,\ x \col R(a,b)\}\subseteq \consis{\qelemg}$ since $\langle \qelemg, x, \qelemg', x, R\rangle\notin\rolesf$ for some $\qelemg'\in\Delta$ with $(x'\col b)\in\consis{\qelemg'}$.

            First, notice that, since $\mathbf{CG}$ is produced by the tableau algorithm, there is exactly one element $\qelemg\in\Delta$ with $(x\col a)\in\consis{\qelemg}$ and one element $\qelemg'\in\Delta$ with $(x'\col b)\in\consis{\qelemg'}$ (see the initialisation of the tableau and its rules \Cref{fig:rules}). Moreover, by the definition of a quasi-model, there is also exactly one element $\qelem\in\Delta^q$ with $(x\col a)\in\consisq{\qelem}$ and one element $\qelem'\in\Delta^q$ with $(x'\col b)\in\consisq{\qelem'}$. From this and the construction of $\crel$, we have only two pairs $(\qelemg,\qelem),(\qelemg',\qelem')\in\crel$ related to this rule.

            Let $y$ be a variable in $\consisq{\qelem}$ such that $\cfunc{\qelemg,\qelem}{y} = x$. Then we have $\{y\col a,\ y\col R(a,b)\}\subseteq\consisq{\qelem}$. By the non-applicability of the  $\mathbf{R}_{r}$ rule, we also have $\langle \qelem, y, \qelem', y, R\rangle\in\rolesf^q$. And, by the definition of a completion graph $\stlabel{\qelem}{y}=\stlabel{\qelem'}{y}$.
            Thus we have $\{y \col \top\}\ \cup\ \{y\col \st \mid \st\in\stlabel{\qelem}{y} \}\subseteq\consis{\qelem'}$ and $\rolesf:=\rolesf\cup \{\langle \qelem, y, \qelem', y, R\rangle\}$.

            By the application of $\mathbf{R}_{r}$ on $\mathbf{CG}$, we obtain $\langle \qelemg, x, \qelemg', x, R\rangle\in\rolesf$ and $\{x \col \top\}\ \cup\ \{x\col \st \mid \st\in\stlabel{\qelemg}{x} \}\subseteq\consis{\qelemg'}$ and $\rolesf:=\rolesf\cup \{\langle \qelemg, x, \qelemg', x, R\rangle\}$.
            Then we define $\cfuncfp{\qelemg',\qelem'}$ as the update of $\cfuncf{\qelemg',\qelem'}$ with $\cfuncp{\qelemg',\qelem'}{y} = x$. Hence, the relation $\crel$ and the functions $\cfuncfp{\qelemg',\qelem'}$ and $\cfuncf{\qelemg,\qelem}$ are as required for the resulting completion graph $\mathbf{CG}'$.

        \item[$\mathbf{R}_{r'}\ $]
            Suppose that the rule $\mathbf{R}_{r'}$ is applicable to the constraints $\{x \col b,\ x \col R(a,b)\}\subseteq \consis{\qelemg}$ since $\langle \qelemg', x, \qelemg, x, R\rangle\notin\rolesf$ for some $\qelemg'\in\Delta$ with $(x'\col a)\in\consis{\qelemg'}$.

            First, notice that, since $\mathbf{CG}$ is produced by the tableau algorithm, there is exactly one element $\qelemg\in\Delta$ with $(x\col b)\in\consis{\qelemg}$ and one element $\qelemg'\in\Delta$ with $(x'\col a)\in\consis{\qelemg'}$ (see the initialisation of the tableau and its rules \Cref{fig:rules}). Moreover, by the definition of a quasi-model, there is also exactly one element $\qelem\in\Delta^q$ with $(x\col b)\in\consisq{\qelem}$ and one element $\qelem'\in\Delta^q$ with $(x'\col a)\in\consisq{\qelem'}$. From this and the construction of $\crel$, we have only two pairs $(\qelemg,\qelem),(\qelemg',\qelem')\in\crel$ related to this rule.

            Let $y$ be a variable in $\consisq{\qelem}$ such that $\cfunc{\qelemg,\qelem}{y} = x$. Then we have $\{y\col b,\ y\col R(a,b)\}\subseteq\consisq{\qelem}$. By the non-applicability of the  $\mathbf{R}_{r'}$ rule, we also have $\langle \qelem', y, \qelem, y, R\rangle\in\rolesf^q$. And, by the definition of a completion graph $\stlabel{\qelem}{y}=\stlabel{\qelem'}{y}$.
            Thus we have $\{y \col \top\}\ \cup\ \{y\col \st \mid \st\in\stlabel{\qelem}{y} \}\subseteq\consis{\qelem'}$ and $\rolesf:=\rolesf\cup \{\langle \qelem', y, \qelem, y, R\rangle\}$.

            By the application of $\mathbf{R}_{r'}$ on $\mathbf{CG}$, we obtain $\langle \qelemg', x, \qelemg, x, R\rangle\in\rolesf$ and $\{x \col \top\}\ \cup\ \{x\col \st \mid \st\in\stlabel{\qelemg}{x} \}\subseteq\consis{\qelemg'}$ and $\rolesf:=\rolesf\cup \{\langle \qelemg', x, \qelemg, x, R\rangle\}$.
            Then we define $\cfuncfp{\qelemg',\qelem'}$ as the update of $\cfuncf{\qelemg',\qelem'}$ with $\cfuncp{\qelemg',\qelem'}{y} = x$. Hence, the relation $\crel$ and the functions $\cfuncfp{\qelemg',\qelem'}$ and $\cfuncf{\qelemg,\qelem}$ are as required for the resulting completion graph $\mathbf{CG}'$.

        \item[$\mathbf{R}_{\exists'}\ $] Suppose that the rule $\mathbf{R}_{\exists'}$ is applicable to a constraint $(x \col \exists R.C)\in \consis{\qelemg}$ for which there is a $\qelemg'$ with $(C,\stlabel{\qelemg}{x},x')\in\elabel{\qelemg'}$ and $\qelemg\neq\qelemg'$, since $\langle \qelemg, x, \qelemg'', x'', R\rangle\notin\rolesf$ for some $\qelemg'', x''$ with $(x'' \col C)\in \consis{\qelem''}$.%, then set $\rolesf:=\rolesf\cup \{\langle \qelem, x, \qelem', x', R\rangle\}$.

            Let $(\qelemg,\qelem)\in\crel$, let $y$ be a variable in $\consisq{\qelem}$ such that $\cfunc{\qelemg,\qelem}{y} = x$. Then we have $(y \col \exists R.C)\in \consis{\qelem}$, and by the non-applicability of the $\mathbf{R}_{\exists'}$ rule to $\mathcal{Q}$, there must be some $\langle \qelem, y, \qelem', y', R\rangle\in\rolesf^q$ for some $\qelem', y'$ with $(C,\stlabel{\qelem}{y},y')\in\elabel{\qelem'}$.
            By the application of the $\mathbf{R}_{\exists'}$ rule on $\mathbf{CG}$, we obtain $\rolesf:=\rolesf\cup \{\langle \qelemg, x, \qelemg', x', R\rangle\}$. Then the relation $\crel$ and the functions $\cfuncfp{\qelemg',\qelem'}$ and $\cfuncf{\qelemg,\qelem}$ are as required for the resulting completion graph $\mathbf{CG}'$.

            Specifically notice that since $\langle \qelemg, x, \qelemg', x', R\rangle\in\rolesf$ there must be some $(\qelemg,\qelem), (\qelemg',\qelem')\in\crel$ with $\cfunc{\qelemg,\qelem}{y}=x$ and $\cfunc{\qelemg',\qelem'}{y'}=x'$ and $\tuple{\qelem, y, \qelem', y', R}\in\rolesf^q$. We already have that $(\qelemg,\qelem)\in\crel$ and $\cfunc{\qelemg,\qelem}{y} = x$. Moreover, by the $\mathbf{R}_{\exists}$ rule we have that for all $\qelemg''$ with $(C,\stlabel{\qelemg}{x},x')\in\elabel{\qelemg''}$ and all $\qelem''$ with $(C,\stlabel{\qelem}{y},y')\in\elabel{\qelem''}$, $(\qelemg'',\qelem'')\in\crel$. Thus we have $(\qelemg',\qelem')\in\crel$. Moreover, we also know from the application of the $\mathbf{R}_{\exists}$ rule that $\cfunc{\qelemg',\qelem'}{y'} = x'$. Hence there are some $(\qelemg,\qelem), (\qelemg',\qelem')\in\crel$ with $\cfunc{\qelemg,\qelem}{y}=x$ and $\cfunc{\qelemg',\qelem'}{y'}=x'$ such that $\langle \qelem, y, \qelem', y', R\rangle\in\rolesf^q$ as required.

    \end{description}
    \vspace{0.5em}

    With this, the claim is proved.
    \vspace{1.5em}

    Now, returning to the proof of the completeness theorem, we show that it
    follows from the claims above. Notice that $\mathbf{CG}_{\kb}$ is the initial completion graph produced by the algorithm for $\kb$ and that we have shown that it is $\mathcal{Q}$-compatible.
    By the second claim, the completion rules can be applied in such a way that
    the resulting completion graphs are $\mathcal{Q}$-compatible. According to Theorem \ref{theorem:termination} (Termination), we then eventually construct a globally complete $\mathcal{Q}$-compatible completion graph $\mathbf{CG}$.

    Let us now show that $\mathbf{CG}$ is coherent. For the first point, we may just observe that we initialise the algorithm with a unique element $\qelem_a\in\Delta$ for each $a\in\objC$ such that $(v_{*}\col a)\in\consisu{\qelem_a}$. Moreover, by the non-applicability of the $\mathbf{R}_{\downarrow}$ rule, we have that $(v\col a)\in\consisu{\qelem_a}$ for all variables $v$ in $\consisu{\qelem_a}$. Since no rule in \Cref{fig:rules} can propagate constraints of the form $(v\col a)$ to other elements, the first condition is satisfied. For the second condition, from \Cref{lemma:same-standpoints} it follows that for each $v$ in $\consis{\qelem}$, every $\consis{\qelem'}$ contains some $v'$ such that $\stlabel{\qelem}{v}=\stlabel{\qelem'}{v'}$ as desired. Finally, from \Cref{lemma:same-axiom-per-standpoint} it follows that for each $\consis{\qelem}$ and $\consis{\qelem'}$, if $(v\col\phi)\in\consis{\qelem}$ then $(v'\col\phi)\in\consis{\qelem'}$ for all $v'$ with $\stlabel{\qelem}{v}=\stlabel{\qelem'}{v'}$ as desired and we can thus conclude that $\mathbf{CG}$ is coherent.

    It remains to show that $\mathbf{CG}$ is clash-free. Suppose otherwise. Then there is an element $\qelemg$ in $\mathbf{CG}$ and a variable $x$ such that $(x\col\bot)\in\consis{\qelemg}$. Let $\crel$ be the relation supplied by the definition of $\mathcal{Q}$-compatibility. Then we must have some $\qelem\in\Delta^q$ with $(\qelemg,\qelem)\in\crel$ and some function $\cfuncf{\qelemg,\qelem}$ such that $(\cfunc{\qelemg,\qelem}{x}\col\bot)\in\consisq{\qelem}$, which is a contradiction because $\mathcal{Q}$ is a quasi-model.
\end{proof}
\subsection{Examples}

\subsubsection{Example of element labels}

\begin{align*}
    C & \sqsubseteq \exists R.D  \\
    D & \sqsubseteq \allstandd C \\
    a & : D
\end{align*}

\begin{tikzpicture}

    \vismprec{4}{12}{$v_*$}
    \visprec{3}{12}{$\pi_1$}
    \visprec{2}{12}{$\pi_2$}
    \visprec{1}{12}{$\pi_3$}

    \visqelem{1}{6}{$(*,a)$}
    \visqelem{7}{6}{$(\pi_2,D)$}

    \vispoint{1}{4}{$D,\allstandd C$}
    \vispoint{1}{3}{$D,\allstandd C,C,\exists R.D$}

    \vispoint{7}{4}{$\top$}
    \vispoint{7}{2}{$D,\allstandd C$}
    \vispoint{7}{1}{$C,\exists R.D$}

\end{tikzpicture}
\newpage
\subsubsection{Easy example of element labels}

\begin{align*}
    C & \sqsubseteq \exists R.D  \\
    \standbs [a & : \standds C ]
\end{align*}

\begin{tikzpicture}

    \vismprec{4}{12}{$v_*$}
    \vismprec{3}{12}{$v_{\st}$}
    \visprec{2}{12}{$v_1$}
    \visprec{1}{12}{$v_2$}

    \visqelem{1}{6}{$(a)$}
    \visqelem{7}{6}{$(D,\st,v_2)$}

    \vispoint{1}{4}{$a$}
    \vispoint{1}{3}{$a, \st, \standds C$}
    \vispoint{1}{2}{$\st, C, a, \exists R.D$}

    \vispoint{7}{4}{$\top$}
    \vispoint{7}{3}{$\top,\st$}
    \vispoint{7}{1}{$\st, D$}

\end{tikzpicture}
\subsubsection{harder example of element labels}

\begin{align*}
    C & \sqsubseteq \exists R.D  \\
    D & \sqsubseteq \standds C \\
    a & : D
\end{align*}

\begin{tikzpicture}

    \vismprec{6}{12}{$v_*$}
    \visprec{5}{12}{$\pi_1$}
    \visprec{4}{12}{$\pi_2$}
    \visprec{3}{12}{$\pi_3$}
    \visprec{2}{12}{$\pi_4$}
    \visprec{1}{12}{$\pi_5$}
    

    \visqelem{1}{8}{$(a)$}
    \visqelem{5}{8}{$(C,\st,\pi_2)$}
    \visqelem{9}{8}{$(C,\st,\pi_4)$}

    \vispoint{1}{6}{$a, D,\standds C$}
    \vispoint{1}{5}{$\st, C, a, D,\standds C, \exists R.D$}

    \vispoint{5}{6}{$\top$}
    \vispoint{5}{4}{$\st, D,\standds C$}
    \vispoint{5}{3}{$\st, C,\exists R.D$}

    \vispoint{9}{6}{$\top$}
    \vispoint{9}{2}{$\st, D,\standds C$}
    \vispoint{9}{1}{$\st, C,\exists R.D$}

\end{tikzpicture}


\begin{align*}
    \top       & \sqsubseteq \exists R.A  \\
    A          & \sqsubseteq \allstandd B \\
    A \sqcap B & \sqsubseteq \bot
\end{align*}

\begin{tikzpicture}

    \visqelem{1}{6}{$(*,\top)$}
    \vismprec{4}{12}{$v_*$}
    \vispoint{1}{4}{$\exists R.A$}
    % Create new element
    \visqelem{5}{6}{$(A,*,\mathbf{t})$}
    \vispoint{5}{4}{$A, \allstandd B, \exists R.A$}
    % Create new precisification
    \visprec{3}{12}{$\pi_1$}
    \vispoint{5}{3}{$A, B, \exists R.A, \bot $}
    % Create new element
    \visqelem{9}{6}{$(A,*,\mathbf{f})$}
    \visprec{2}{12}{$\pi_2$}
    \vispoint{9}{4}{$\exists R.A$}
    \vispoint{9}{2}{$A, \allstandd B, \exists R.A$}


    % \visprec{2}{12}{$\pi_2$}
    % \visprec{1}{12}{$\pi_3$}



    % \vispoint{7}{4}{$\top$}
    % \vispoint{7}{2}{$D,\allstandd C$}
    % \vispoint{7}{1}{$C,\exists R.D$}

\end{tikzpicture}


\begin{align*}
    \top        & \sqsubseteq \exists R.A \\
    A           & \sqsubseteq B           \\
    \exists R.B & \sqsubseteq \bot
\end{align*}

\begin{tikzpicture}

    \visqelem{1}{6}{$(*,\top)$}
    \vismprec{4}{12}{$v_*$}
    \vispoint{1}{4}{$\exists R.A$}
    % Create new element
    \visqelem{5}{6}{$(A,*,\mathbf{t})$}
    \vispoint{5}{4}{$A, \allstandd B, \exists R.A$}
    % Create new precisification
    \visprec{3}{12}{$\pi_1$}
    \vispoint{5}{3}{$A, B, \exists R.A, \bot $}
    % Create new element
    \visqelem{9}{6}{$(A,*,\mathbf{f})$}
    \visprec{2}{12}{$\pi_2$}
    \vispoint{9}{4}{$\exists R.A$}
    \vispoint{9}{2}{$A, \allstandd B, \exists R.A$}


\end{tikzpicture}


\subsubsection{Example of the need to set up fancier runs for the existential rule in boxes}

\begin{align*}
    \top & \sqsubseteq \exists R.A \\
\end{align*}

\begin{tikzpicture}

    \visqelem{1}{4}{$(*,\top)$}
    \visqelem{5}{4}{$(A,*)$}

    \vismprec{2}{8}{$v_*$}
    \visprec{1}{8}{$\pi_1$}

    \vispoint{1}{2}{$\exists R.A$}
    \vispoint{5}{2}{$\exists R.A$}

    \vispoint{5}{1}{$A, \exists R.A$}

\end{tikzpicture}

Note that there is no run for $v_{*}$ in the second qelement. When we set up the runs  we need to duplicate each qelement, so alternative ones can be chosen.
\newpage

\begin{align*}
    \top & \sqsubseteq  A           \\
    \top & \sqsubseteq \exists R.A  \\
    A    & \sqsubseteq \allstandd B
\end{align*}

\begin{tikzpicture}

    \visqelem{1}{6}{$\emptyset$}
    \visqelem{5}{6}{$(A,*)$}

    \vismprec{4}{8}{$v_*$}
    \visprec{3}{8}{$\pi_1$}
    \visprec{2}{8}{$\pi_2$}
    \visprec{1}{8}{$\pi_3$}

    \vispoint{1}{4}{$A, \exists R.A, \allstandd B$}
    \vispoint{1}{3}{$B, A, \exists R.A, \allstandd B$}

    \vispoint{5}{4}{$A, \exists R.A, \allstandd B$}
    \vispoint{5}{2}{$A, \exists R.A, \allstandd B$}
    \vispoint{5}{1}{$B, A, \exists R.A, \allstandd B$}

\end{tikzpicture}

Maybe check the following two examples:

\begin{align*}
    \top        & \sqsubseteq \allstandd A \\
    A           & \sqsubseteq \exists R.B  \\
    B           & \sqsubseteq  C           \\
    \exists R.C & \sqsubseteq \bot         \\
\end{align*}

\begin{align*}
    \top        & \sqsubseteq \exists R.B \\
    B           & \sqsubseteq  C          \\
    \exists R.C & \sqsubseteq \bot        \\
\end{align*}
\newpage
\subsubsection{Example of existentials on named individuals}

\begin{align*}
    \top        & \sqsubseteq C            \\
    C           & \sqsubseteq \allstandd D \\
    \exists R.D & \sqsubseteq \bot         \\
    R           & (a,b)
\end{align*}

\begin{tikzpicture}

    \visqelem{1}{6}{$(a)$}
    \visqelem{5}{6}{$(b)$}

    \vismprec{4}{8}{$v_*$}
    \visprec{3}{8}{$\pi_1$}
    \visprec{2}{8}{$\pi_2$}
    \visprec{1}{8}{$\pi_2$}

    \vispoint{1}{4}{$C, \allstandd D$}
    \vispoint{5}{4}{$C, \allstandd D$}

    \vispoint{1}{3}{$C, \allstandd D, D$}
    \vispoint{5}{2}{$C, \allstandd D, D$}

    \vispoint{1}{1}{$C, \allstandd D, \exists R.D, \bot$}

\end{tikzpicture}

\subsubsection{Example}

\begin{align*}
    \top         & \sqsubseteq C           \\
    \allstandd C & \sqsubseteq D           \\
    \top         & \sqsubseteq \exists R.E \\
\end{align*}

\begin{tikzpicture}

    \visqelem{1}{6}{$(\top)$}
    \visqelem{5}{6}{$(E, *, \pi_2)$}
    \visqelem{9}{6}{$(E, *, \pi_2)_c$}

    \vismprec{4}{13}{$v_*$}
    \visprec{3}{13}{$\pi_1$}
    \visprec{2}{13}{$\pi_2$}
    \visprec{1}{13}{$\pi_2$}

    \vispoint{1}{4}{$C, \exists R.E$}
    \vispoint{1}{3}{$C, C\sqsubseteq D, D, \exists R.E$}

    \vispoint{5}{4}{$C, \exists R.E$}
    \vispoint{5}{2}{$C, E, \exists R.E$}
    \vispoint{5}{1}{$C, D, C\sqsubseteq D, \exists R.E$}

    \vispoint{9}{4}{$C, \exists R.E$}
    \vispoint{9}{2}{$C, E, \exists R.E$}
    \vispoint{9}{1}{$C, D, C\sqsubseteq D, \exists R.E$}

\end{tikzpicture}

\subsubsection{Example of existentials without named individuals}

\begin{align*}
    \top        & \sqsubseteq C            \\
    C           & \sqsubseteq \allstandd D \\
    \exists R.D & \sqsubseteq \bot         \\
    \top        & \sqsubseteq \exists R.E  \\
\end{align*}

\begin{tikzpicture}

    \visqelem{1}{6}{$(\top)$}
    \visqelem{5}{6}{$(E, *, \pi_2)$}
    \visqelem{9}{6}{$(E, *, \pi_2)_c$}

    \vismprec{4}{13}{$v_*$}
    \visprec{3}{13}{$\pi_1$}
    \visprec{2}{13}{$\pi_2$}
    \visprec{1}{13}{$\pi_2$}

    \vispoint{1}{4}{$C, \allstandd D, \exists R.E$}
    \vispoint{1}{3}{$C, \allstandd D, D, \exists R.E$}

    \vispoint{5}{4}{$C, \allstandd D, \exists R.E$}
    \vispoint{5}{2}{$C, E, \allstandd D, \exists R.E$}
    \vispoint{5}{1}{$C, D, \allstandd D, \exists R.E$}

    \vispoint{9}{4}{$C, \allstandd D, \exists R.E$}
    \vispoint{9}{2}{$C, E, \allstandd D, \exists R.E$}
    \vispoint{9}{1}{$C, D, \allstandd D, \exists R.E$}

\end{tikzpicture}

Runs:
\begin{itemize}
    \item \bf r(1)= (1,1)\sf; r(2)= (2,3); r(3)= (3,1); $R(1,2)$, $R(2,2)$, $R(3,2)$
    \item \bf r(1)= (1,2)\sf; r(2)= (2,3); r(3)= (3,1); $R(1,2)$, $R(2,2)$, $R(3,2)$
    \item r(1)= (1,1); \bf r(2)= (2,1)\sf; r(3)= (3,3); $R(1,3)$, $R(2,3)$, $R(3,3)$
    \item \dots
\end{itemize}

==> sections/proofs-section-4.tex <==
    \begin{theorem}
        Satisfiability of $\SEL$ TBoxes with $*$ as the only occurring standpoint name and one distinguished rigid role $\dot{R}$ is \coNP-hard.
        \begin{proof}
            We reduce the \NP-hard problem SAT to TBox unsatisfiability.
            Assume an instance $\phi=\clause_1 \land \ldots \land \clause_n$ of SAT containing $n$ clauses $\clause_j$ (disjunctions of literals) over the propositional variables \mbox{$P = \set{ p_1,\ldots, p_k }$}.

            We construct the following $\SELO$ TBox $\T_\phi$ (of polynomial size):
            \begin{align}
                \top                                                  & \sqsubseteq \exists U. L_0                                                                                                                    \label{lstart}                                                                                    \\
                L_{i-1}                                               & \sqsubseteq \exists \dot{R}.(T_{p_i} \sqcap L_{i} ) \sqcap \exists \dot{R}. (T_{\neg p_i} \sqcap L_{i})                                                      & \text{ for all } 1\leq i\leq k      \label{lnext}                                \\
                L_{i} \sqcap T_{p_i}                                  & \sqsubseteq \standball ( L_{i} \sqcap T_{p_i} )                                                                                                              & \text{ for all } 1\leq i\leq k                                     \label{ltrue} \\
                L_{i} \sqcap T_{\neg p_i}                             & \sqsubseteq \standball ( L_{i} \sqcap T_{\neg p_i} )                                                                                                         & \text{ for all } 1\leq i\leq k      \label{lfalse}                               \\
                L_k                                                   & \sqsubseteq \standdall\!\mathit{Select}                                                                        \label{sstart}                                                                                                                   \\
                \exists \dot{R}.(T_{p_i} \sqcap \mathit{Select})      & \sqsubseteq (T_{p_i} \sqcap \mathit{Select})                                                                                                                 & \text{ for all } 1\leq i\leq k                       \label{strue}               \\
                \exists \dot{R}.(T_{\neg p_i} \sqcap \mathit{Select}) & \sqsubseteq (T_{\neg p_i} \sqcap \mathit{Select})                                                                                                            & \text{ for all } 1\leq i\leq k  \label{sfalse}                                   \\
                T_\ell                                                & \sqsubseteq T_{\clause_j}                                                                                                                                    & \text{ for all } \ell \in \clause_j \label{clause}                               \\
                T_{\clause_1} \sqcap \ldots \sqcap T_{\clause_n}      & \sqsubseteq \bot  \label{disjoint}
            \end{align}
            We conclude the proof by showing that $\phi$ is satisfiable iff $\T_\phi$ is unsatisfiable.
            \begin{description}
                \item[\normalfont``if'':]
                    We show the contrapositive.
                    Let $\phi$ be unsatisfiable.
                    We construct a model \mbox{$\dlstruct= \tuple{\Dom, \Precs, \sigma, \gamma}$} for $\T_\phi$ as follows.
                    \begin{align*}
                        \Dom   & = \set{ w\in\set{0,1}^* \guard \abs{w}\leq k } \\
                        \Precs & = 2^P
                    \end{align*}
                    That is, the interpretation domain contains all words $w$ over $\set{0,1}$ of length at most $k$ (including the empty word $\nil$).
                    Roughly, each $w$ encodes a partial interpretation of $P$ where $w_i$, the $i$-th symbol in $w$, encodes whether $p_i$ is true ($w_i=1$) or false ($w_i=0$) or undefined ($\abs{w}<i$).

                    Finally, for each $Q\subseteq P$, the DL interpretation $\gamma(Q)=\tuple{\Dom,\intf}$ is given by
                    \begin{align*}
                        \interprets{U}               & = \Dom\times\set{ \nil }                                                                           \\
                        \interprets{\dot{R}}          & = \set{ \tuple{w,w0}, \tuple{w,w1} \guard w,w0,w1\in\Dom }                                         \\
                        \interprets{L_i}             & = \set{ w\in\Dom \guard \abs{w}=i }                                                                \\
                        \interprets{T_{p_i}}         & = \set{ w\in\Dom \guard w_i=1 } \cup \set{ w\in\Dom \guard w\in\prefixes(w^Q), \abs{w}<i, w^Q_i=1} \\
                        \interprets{T_{\neg p_i}}    & = \set{ w\in\Dom \guard w_i=0 } \cup \set{ w\in\Dom \guard w\in\prefixes(w^Q), \abs{w}<i, w^Q_i=0} \\
                        \interprets{\mathit{Select}} & = \prefixes(w^Q)                                                                                   \\
                        \interprets{T_{\clause_j}}   & = \bigcup_{\ell\in\clause_j}\interprets{T_{\ell}}
                    \end{align*}
                    Where the word $w^Q$ of length $k$ encodes the valuation $Q$ via
                    \[
                        w^Q_i               = \begin{cases}
                            0 & \text{ if } p_i\notin Q \\
                            1 & \text{ otherwise}
                        \end{cases}
                    \]
                    and $\prefixes(w)=\set{v\in\set{0,1}^* \guard \exists u\in\set{0,1}^*: w=vu}$ denotes the set of all prefixes of $w\in\set{0,1}^*$.
                    %Observe that $Q\models p_i$ iff $w^Q\in T_{p_i}$, and $Q\not\models p_i$ iff $w^Q\in T_{\neg p_i}$.

                    We now show that $\dlstruct\models\T_\phi$.
                    Unless declared otherwise, assume that $\struct=\gamma(Q)$ is for an arbitrary $Q\subseteq P$.

                    We note that the interpretations of the $L_i$ ($0\leq i\leq k$) and $T_{\clause_j}$ ($1\leq j\leq n$) is the same across precisifications, and for $T_{p_i}$ and $T_{\neg p_i}$ their extensions agree on all words of length at least $i$.
                    \begin{itemize}
                        \item (\ref{lstart}): By definition.
                        \item (\ref{lnext}): Let $w\in\interprets{L_{i-1}}$.
                              Then $\abs{w}=i-1$.
                              In particular, since $i-1<k$, we have $w0,w1\in\Dom$ and thus $\tuple{w,w0},\tuple{w,w1}\in\interprets{\dot{R}}$.
                              Clearly, $\abs{w0}=\abs{w1}=i$ whence $w0,w1\in\interprets{L_i}$.
                              Furthermore, $(w0)_i=0$ whence $w0\in T_{\neg p_i}$;
                              likewise $(w1)_i=1$ and $w1\in T_{p_i}$.
                        \item (\ref{ltrue}): Let $w\in\interprets{L_i}\cap\interprets{T_{p_i}}$.
                              Then $\abs{w}=i$ and $w_i=1$ by definition.
                              Thus by agreement across precisifications, for any $Q\subseteq P$ we get $w\in(L_i\dland T_{p_i})^{\gamma(Q)}$, whence $w\in \bigcap_{Q\subseteq P} (L_i\dland T_{p_i})^{\gamma(Q)}$.
                        \item (\ref{lfalse}): Symmetric.
                        \item (\ref{sstart}): Let $w\in\interprets{L_k}$.
                              Then $\abs{w}=k$ and there is a $Q\subseteq P$ such that $w^Q=w$.
                              Since $w=w^Q\in\prefixes(w^Q)$ by definition, for $\gamma(Q)$ we thus have $w\in (\mathit{Select})^{\gamma(Q)}$.
                        \item (\ref{strue}): Let $\tuple{v,w}\in\interprets{\dot{R}}$ such that $w\in\interprets{T_{p_i}}\cap\interprets{\mathit{Select}}$.
                              Then $w\in\prefixes(w^Q)$, and either
                              (a) $\abs{w}=i$ and $w_i=1$, or
                              (b) $\abs{w}<i$ and $w^Q_i=1$.
                              By definition of $\interprets{\dot{R}}$ we have $v\in\prefixes(w)\subseteq\prefixes(w^Q)$, whence $v\in\interprets{\mathit{Select}}$.
                              In particular, $\abs{v}=i-1<i$ and in any case we have $w^Q_i=1$, thus $v\in\interprets{T_{p_i}}$.
                        \item (\ref{sfalse}): Symmetric.
                        \item (\ref{clause}): By definition.
                        \item (\ref{disjoint}): By contradiction:
                              Assume that there is a $Q\subseteq P$ such that for $\struct=\gamma(Q)$, there is some $w\in\interprets{T_{\clause_1}}\cap\ldots\cap\interprets{T_{\clause_n}}$.
                              Then by definition, for each $1\leq j\leq n$ there is an $\ell_j\in\clause_j$ such that $w\in\interprets{T_{\ell_j}}$.
                              Define $R_w = \set{ p\in P \guard w\in \interprets{T_{p}} } \cup \set{ \neg p \guard p\in P, w\in\interprets{T_{\neg p}}}$.
                              $R_w$ is consistent because for all $1\leq i\leq k$, we have $\interprets{T_{p_i}}\cap\interprets{T_{\neg p_i}}=\emptyset$.
                              We show $R_w\cap P\models\phi$ to obtain the desired contradiction with unsatisfiability of $\phi$.
                              Consider $\clause_j$.
                              We have $\ell_j\in\clause_j$ as above with $w\in\interprets{T_{\ell_j}}$, whence by definition $\ell_j\in R_w$.
                              Consequently, $R_w\cap P\models\ell_j$.
                              Since $\clause_j$ was chosen arbitrarily, we get $R_w\cap P\models\phi$.
                    \end{itemize}
                \item[\normalfont``only if'':]
                    Let $\phi$ be satisfiable.
                    Then there is a $Q\subseteq P$ such that $Q\models\phi$.
                    We show by contradiction that $\T_\phi$ is unsatisfiable.
                    Assume that there is a Standpoint DL structure $\dlstruct=\tuple{\Dom,\Precs,\sigma,\gamma}$ such that $\dlstruct\models\T_\phi$.
                    By $\dlstruct\models (\ref{lstart}) \land (\ref{lnext})$, in every $\pr\in\Precs$, $\dot{R}$ contains a full binary tree of depth $k$ where in each layer $i$, the nodes (individuals $\de_i\in\Dom$) are marked with $L_i$, and one of $T_{p_i}$ and $T_{\neg p_i}$, respectively.
                    Due to the rigid role $\dot{R}$ being used and rigidity of $L_i\dland T_{(\neg)p_i}$ being enforced by (\ref{ltrue}) and (\ref{lfalse}), this part of the interpretation is “the same” across precisifications.
                    Employing $\dlstruct\models (\ref{sstart})$, we now consider $\pr\in\Precs$ and the sequence
                    $\de_0,\ldots,\de_k\in\Dom$ with $\de_0\in\interpretgp{L_0}$,
                    $\tuple{\de_{i-1},\de_i}\in\interpretgp{\dot{R}}$ for all $1\leq i\leq k$,
                    $\de_i\in\interpretgp{L_i}\cap\interpretgp{\mathit{Select}}$ for all $1\leq i\leq k$ such that for all $p_i\in P$:
                    \begin{itemize}
                        \item $\de_i\in\interpretgp{T_{p_i}}$ whenever $p_i\in Q$,
                        \item $\de_i\in\interpretgp{T_{\neg p_i}}$ whenever $p_i\notin Q$.
                    \end{itemize}
                    Since $\dlstruct\models (\ref{lnext}) \land (\ref{strue}) \land (\ref{sfalse})$, it follows that for all $p\in P$:
                    \begin{itemize}
                        \item $\de_1\in\interpretgp{T_{p}}$ whenever $p\in Q$,
                        \item $\de_1\in\interpretgp{T_{\neg p}}$ whenever $p\notin Q$.
                    \end{itemize}
                    Now since $Q\models\phi$, we get that $Q\models\clause_j$ for all $1\leq j\leq k$;
                    that is, for every $\clause_j$ there is a literal $\ell_j\in\clause_j$ such that $Q\models\ell_j$.
                    Now $Q\models\ell_j$ iff $\de_1\in\interpretgp{T_{\ell_j}}$ by the above.
                    Thus, for every $\clause_j$ there is $\ell_j\in\clause_j$ such that $\de_1\in\interpretgp{T_{\ell_j}}$.
                    Thus $\de_1\in T_{\clause_j}$ by $\dlstruct\models (\ref{clause})$.
                    But then, since $\clause_j$ was chosen arbitrarily, we get $\de_1 \in \interpretgp{(T_{\clause_1}\dland\ldots\dland T_{\clause_n})}$ in contradiction to $\dlstruct\models (\ref{disjoint})$.
            \end{description}
        \end{proof}
    \end{theorem}

\begin{definition}
From a normalised Horn-$\mathcal{ALC}$ TBox $\mathcal{T}$, we obtain the target $\SELO$ TBox $\SELO(\mathcal{T})$ by
\begin{itemize}[leftmargin=0.7cm]
\item[(i)] declaring every original concept name as rigid via the axiom $A \sqsubseteq \standball A$ as well as
\item[(ii)] replacing every axiom of the shape $A \sqsubseteq \exists R.B$ by the axiom
\begin{linenomath*}
    $$A \sqsubseteq \standdall ((\exists \mathit{Src}.\{o\}) \sqcap (\exists R.(B \sqcap \exists \mathit{Tgt}.\{o\})))$$
\end{linenomath*}
(introducing two fresh role names $\mathit{Src}$ and $\mathit{Tgt}$), and replacing every axiom of the shape $A \sqsubseteq \forall r.B$ by the two axioms
\begin{linenomath*}
    $$A \sqcap \exists R.\top \sqsubseteq (\exists \mathit{Src}.(\{o\} \sqcap \tilde{B})) \quad\text{and}\quad \exists \mathit{Tgt}.\tilde{B} \sqsubseteq B,$$
\end{linenomath*}
introducing a copy $\tilde{A}$ for every original concept name $A$.
\end{itemize}
\end{definition}
     
     
     \begin{theorem}
      Let $\mathcal{T}$ be a normalised Horn-$\mathcal{ALC}$ TBox. Then, $\mathcal{T}$ and $\SELO(\mathcal{T})$ are equisatisfiable.
    \end{theorem}
    \begin{proof}
        We show equisatisfiability of $\mathcal{T}$ and $\SELO(\mathcal{T})$ by providing constructions to obtain a model of $\mathcal{T}$ from a model of $\mathcal{T}'$ and vice versa.
        Let $\mathcal{I}=(\Dom,\cdot^\mathcal{I})$ be a model of $\mathcal{T}$. Then we construct a model
        $\dlstruct= \tuple{\Dom, \Precs, \sigma, \gamma}$ of $\SELO(\mathcal{T})$ as follows:
        \begin{itemize}
            \item $\Precs = \Roles \times \Dom \times \Dom$ with $\sigma(*) = \Precs$,
            \item pick one arbitrary but fixed $\delta_o \in \Dom$ and let $o^{\gamma(\pi)}=\delta_o$ for all $\pi \in \Precs$,
            \item $A^{\gamma(\pi)}=A^\mathcal{I}$ for all $\pi \in \Precs$, whereas
                  $\tilde{A}^{\gamma((r,\delta_1,\delta_2))}= \{ \delta_o \mid \delta_2 \in A^\mathcal{I}\}$ for $A \in \Concepts$,
            \item $R^{\gamma((r,\delta_1,\delta_2))}=\{(\delta_1,\delta_2)\} \cap R^\mathcal{I}$, while
                  $Src^{\gamma((r,\delta_1,\delta_2))}=\{(\delta_1,\delta_o)\}$ and
                  $Tgt^{\gamma((r,\delta_1,\delta_2))}=\{(\delta_2,\delta_o)\}$.
        \end{itemize}

        \medskip

        For the other direction, let $\dlstruct= \tuple{\Dom, \Precs, \sigma, \gamma}$ be a model of $\SELO(\mathcal{T})$. Then we construct a model $\mathcal{I}=(\Dom,\cdot^\mathcal{I})$ of $\mathcal{T}$ as follows:
        \begin{itemize}
            \item $A^\mathcal{I} = A^{\gamma(\pi)}$ for any $\pi \in \Precs$ (the choice is irrelevant because all $A$ are rigid)
            \item $R^\mathcal{I} = \bigcup_{\pi \in \Precs}\{(\delta_1,\delta_2) \in R^{\gamma(\pi)} \mid (\delta_1,o^{\gamma(\pi)}) \in  Src^{\gamma(\pi)},\ (\delta_2,o^{\gamma(\pi)}) \in Tgt^{\gamma(\pi)}\}$
        \end{itemize}
    \end{proof}

